On Agnostic PAC Learning using $\mathcal{L}_2$-polynomial Regression and Fourier-based Algorithms

We develop a framework using Hilbert spaces as a proxy to analyze PAC learning problems with structural properties. We consider a joint Hilbert space incorporating the relation between the true label and the predictor under a joint distribution $D$. We demonstrate that agnostic PAC learning with 0-1 loss is equivalent to an optimization in the Hilbert space domain. With our model, we revisit the PAC learning problem using methods based on least-squares such as $\mathcal{L}_2$ polynomial regression and Linial's low-degree algorithm. We study learning with respect to several hypothesis classes such as half-spaces and polynomial-approximated classes (i.e., functions approximated by a fixed-degree polynomial). We prove that (under some distributional assumptions) such methods obtain generalization error up to $2opt$ with $opt$ being the optimal error of the class. Hence, we show the tightest bound on generalization error when $opt\leq 0.2$.

==> FourierFramework.tex <==
\section{ A Fourier-Based Framework}\label{sec:Fourier Framework}
The Fourier expansion on the Boolean cube has been  a powerful tool to characterize non-linear relations among the features and the labels. \addvc{ Such an  expansion has been developed also on the Boolean cube with non-uniform distribution \citep{ODonnell2014}.  In what follows we present an overview of this Fourier expansion. A more detailed discussion on the properties of this Fourier expansion is available in Appendix \ref{app:Fourier_analysis}. }

\paragraph{The Fourier expansion on the Boolean cube:}
\addvc{ Let $\bfX = (X_1, X_2, ..., X_d)$ be a vector of mutually independent random variables on the Boolean cube $\pmm^d$.  }
Let $\mu_j$ and $\sigma_j$ be the mean and standard-deviation of $X_j, j\in [d]$. Suppose that these random variables are non-trivial, that is $\sigma_j>0$ for all $j\in [d]$. The Fourier expansion is defined via a set of basis functions called \textit{parities}.  The \textit{parity} for a subset $\mathcal{S}\subseteq [d]$ 
is a function $\pS: \RR^d\mapsto \RR$ defined as  
$$\pS(\bfx)\deq \prod_{i\in \mathcal{S}}\frac{x_i-\mu_i}{\sigma_i}, \quad \forall \bfx\in \RR^d.$$
By construction, the above parities are orthonormal. In other words, $\EE[\pS(\bfX)~ \psi_{\mathcal{T}}(\bfX)]=0$ for $\mathcal{S}\neq \mathcal{T}$ and $\EE[ \pS(\bfX)^2]=1$.

 It is known that these parity functions form an orthonormal basis for the space of bounded functions on the Boolean cube \citep{ODonnell2014}, that is when $\mathcal{X}=\pmm^d$.  As a result, any bounded function $f:\pmm^d \mapsto \RR$ can be written as a linear combination of the form 
\begin{align*}%\label{eq:Boolean Fourier}
 f(\bfx)=\sum_{\mathcal{S}\subseteq [d]} \fS~\ps(\bfx), \quad \forall \bfx\in \pmm^d,
\end{align*}
where $\fS\in \RR$ are called the {\it Fourier coefficients} of $f$.  Due to the orthogonality 
of the parities,  the Fourier coefficients can be computed as follows
\begin{align}\label{eq:Fourier coeffs}
 \fS= \EE[f(\bfX)\pS(\bfX)], \quad \forall \mathcal{S}\subseteq [d].
 \end{align}
 \addvc{
 As a special case, the standard Fourier expansion on the Boolean cube is obtained when $X_j$'s are uniform random variables over $\pmm$. As a result, $\pS\equiv \bfx^{\mathcal{S}}$ and $f\equiv \sum_{\mathcal{S}\subseteq [d]} \fS~\bfx^{\mathcal{S}}$.}
%\addva{However, for non-binary input set $\mathcal{X}$, the parities are no longer forming a basis. In this case, the parities span only a subspace of the functions; those of the form $f\equiv \sum_{\mathcal{S}\subseteq [d]}\alpha_{\mathcal{S}} \pS$, where $\alpha_{\mathcal{S}}\in \RR$ for all $\mathcal{S}\subseteq [d]$. Note that the dimension of this space is $2^d$. When $\mathcal{X}=\pmm^d$, this subspace contains all functions on $\mathcal{X}$. Due to the orthonormality of the parities any function $f$ in this subspace has a unique linear decomposition with coefficients $\fS$ as in \eqref{eq:Fourier coeffs}. %In this paper, unless otherwise stated, it is assumed that any function on $\mathcal{X}$ belongs to $\Hspaced$.}
%\begin{definition} \label{def:parity threshold}
%Given the input set $\mathcal{X}\subseteq \RR^d$, a function $g:\mathcal{X}\mapsto \pmm$ is called a \textit{monomial-threshold} function if 
%\begin{align*}
%g(\bfx) = \sign\big[\sum_{\mathcal{S}\subseteq [d]}\alpha_{\mathcal{S}} \bfx^{\mathcal{S}} \big],\qquad \forall \bfx\in\mathcal{X},
%\end{align*}
%where $\bfx^{\mathcal{S}}=\prod_{j\in \mathcal{S}}x_j$, and $\alpha_{\mathcal{S}}\in \RR$ for all $\mathcal{S}\subseteq [d]$. The set of all such functions is denoted by $\Hspaced$.
%\end{definition}
%Using the Fourier expansion, for any bounded function $f\in \Hspaced$ and any 
%subset $\mathcal{J}\subseteq [d]$, we define the {\it projection} of $f$ onto 
%$\mathcal{J}$ as the following real-valued function
%\begin{align}\label{eq:projection J}
% \fJ(\bfx)=\sum_{S\subseteq \mathcal{J}} \fS~\ps(\bfx), \quad \text{for all } \bfx\in \mathcal{X}.
% \end{align} 
%As a special case, for $\mathcal{J}=[d]$, the projection $\fJ$ equals to $f$ itself. For more details on the properties of the Fourier expansion see Appendix \ref{app:Fourier_analysis}.
%In the binary setting, any function is a monomial-threshold function. Further, any \textit{linear-threshold} function is in $\Hspaced$. 


==> Fourier_based_learning.tex <==
\section{Fourier-Based Learning Algorithm}\label{sec:Fourier Learning }

We build upon the characterization of optimal 
predictor (Proposition \ref{prop:kjunta_nonbinary}) and  propose a 
Fourier-based supervised learning algorithm with an embedded feature 
selection (see Algorithm \ref{alg:feature_selection}). In \textit{agnostic} PAC learning, a learning algorithm achieves the minimum attainable misclassification probability under any feature-label distribution. In this paper, our theoretical guarantees hold under the condition that the features are independent. To emphasize this, we first present a notion of \textit{agnostic} PAC learning which is restricted to a class of feature-label distributions. 


%\addvb{Due to the hardness results such as \citep{Kearns1994,Guruswami2006} and \citep{Lee1995} for agnostic learning under general distributions,  we introduce a distribution-specific formulation for agnostic PAC learning.}

 \begin{definition} [$\mathscr{P}$-Universality]\label{def:universal_alg} 
Given a class of feature-label distribution $\mathscr{P}$, a learning algorithm is said to be universal, 
if it agnostically learns with respect to a hypothesis class $\mathcal{H}$ under any feature distribution $P_{\bfX,Y}\in \mathscr{P}$. More precisely, for every $\epsilon, \delta \in (0,1)$, every probability 
distribution $P_{\bfX,Y}\in \mathscr{P}$, 
and at least $n(\epsilon,\delta)$ number of \ac{IID} training samples 
generated by $P_{\bfX,Y}$, the algorithm produces,  
with probability at least $(1-\delta)$, a hypothesis $g\in \mathcal{H}$ with 
misclassification probability at most $\Popt+\epsilon$.
\end{definition}

%This definition implies that the feature subset generated by a universal algorithm is ``almost optimal" in terms of misclassification rate. In other words, even if the labeling function $f$ and the feature's probability distribution $P_{\bfX}$  were known to any learning algorithm, the misclassification rate would be almost equal to that of a universal algorithm.  
The focus of this section is on $\mathscr{P}$-universality with  $\mathscr{P}$ being the set of all $P_{\bfX,Y}$ on $\pmm^d\times \pmm$ such that the marginal  $P_{\bfX}$ is a product probability distribution and $Y=f(\bfX)$ for some unknown function $f$. Further, the hypothesis class is the set of all functions $g$ that depends on at most $k$ inputs. \addvb{In section \ref{sec:stochastic} we extend our result to stochastic labeling, that is when the label is generated according to an unknown, but fixed, conditional probability distribution $P_{Y|\bfX}$. }  





\section{Extensions to Stochastic Labeling}\label{sec:stochastic}
The Fourier framework in Section \ref{sec:Fourier Framework} is developed for deterministic labeling, where $Y=f(\bfX)$ for some function $f$. In this section, we address this restriction and extend the Fourier framework to stochastic mappings. We show that our results in Proposition \ref{prop:kjunta_nonbinary},  Theorem \ref{thm:unknownf_and_D}, and \ref{thm:regret}  still hold when the labels are generated according to an arbitrary unknown probability distribution $P_{Y|\bfX}$. More precisely, based on Definition \ref{def:universal_alg}, we consider $\mathscr{P}$-universal learning where $\mathscr{P}$ is the set of all distributions $P_{\bfX,Y}$ on $\pmm^d\times \pmm$ such that $P_{\bfX}$ is a product probability distribution.

In what follows, we prove necessary statements enabling us to extend our Fourier framework to stochastic mappings. We start with generalizing  our notion of projection given in Definition \ref{def:projection Y onto J}.  

\begin{definition}[ \textbf{Projection onto a subset}]\label{def:projection onto J stochastic}
Given a joint probability distribution $P_{\bfX,Y}$ on $\pmm^d\times \pmm$, the projection of $Y$ onto a subset $\mathcal{J}\subseteq [d]$ is defined as 
\begin{align*}
\fJ(\bfx)\deq \sum_{\mathcal{S}\subseteq \mathcal{J}} \EE[Y\pS(\bfX)] \pS(\bfx), \qquad \forall \bfx \in \pmm^d.
\end{align*}
\end{definition}
When $Y$ is a deterministic function of the features $\bfX$, then the above notions reduces to the one in Definition \ref{def:projection Y onto J}. In the following lemma, we show that the projection function $\fJ$ provides a proxy to analyze the misclassification probability.
\begin{lem}\label{lem:pe for stochastic}
Given any subset $\mathcal{J}\subseteq [d]$, let $g:\pmm^d\mapsto\pmm$ be a function whose output depends only on the coordinates of $\mathcal{J}$. Then $
\EE[Y~ g(\bfX)] = \<\fJ, g\>,$ where $\fJ$ is the projection of $Y$ onto $\mathcal{J}$ as in Definition \ref{def:projection onto J stochastic}. Further, the resulted misclassification probability satisfies  
\begin{align}\label{eq:pe for stochastic}
\prob{Y\neq g(\bfX)} &= \frac{1}{2}-\frac{1}{2}~\<\fJ, g\>= \frac{1}{4} \big( \norm{\fJ-g}_2^2 + 1 - \norm{\fJ}_2^2\big).
\end{align}
\end{lem}
\begin{proof}
Since $g$ depends only on $\bfx^{\mathcal{J}}$, then, from Fact \ref{fact:2norm and fJ}, its Fourier expansion is of the form ${g}\equiv \sum_{\mathcal{S}\subseteq\mathcal{J}} g_{\mathcal{S}} \pS$, where $g_{\mathcal{S}}$'s are the Fourier coefficients.  Using this summation we have
\begin{align}\label{eq:correlation YgJ}
\EE[Yg(\bfX)] = \sum_{\mathcal{S}\subseteq\mathcal{J}} g_{\mathcal{S}} ~ \EE[Y\pS(\bfX)] = \sum_{\mathcal{S}\subseteq\mathcal{J}} \EE[{g}(\bfX) \pS(\bfX)] ~ \EE[Y\pS(\bfX)] = \<\fJ,g\>. 
   \end{align}   
   where the second equality holds as $g_{\mathcal{S}} = \<{g},\pS\>$. Hence, the first statement of the lemma is proved. Next, we prove the equalities in \eqref{eq:pe for stochastic}. 
Since $Y$ and $g(\bfX)$ take values from $\pmm$, then 
\begin{align*}
\prob{Y\neq g(\bfX)} &= \frac{1}{2}-\frac{1}{2}~\EE[Yg(\bfX)].
\end{align*}
Hence, with the above equation and \eqref{eq:correlation YgJ}, we establish the first equality in \eqref{eq:pe for stochastic}. Next, we prove the second equality. Form the definition of $2$-norm, we have 
   \begin{align*}
\norm{\fJ-g}_2^2 =\<(\fJ-g), (\fJ-g)\> = \norm{\fJ}_2^2 + \norm{g}_2^2 -2~\<\fJ, g\>.
   \end{align*}
   Since the range of $g$ belongs to $\pmm$, then $\norm{g}_2^2=1$. Therefore, by rewriting the above equality we have 
   \begin{align*}
   \<\fJ, g\> = \frac{1}{2}\big( 1+\norm{\fJ}_2^2-\norm{\fJ-g}_2^2\big).
   \end{align*}
   The proof is complete as this equation implies the second equality in the statement of the lemma. 
\end{proof}

Using this lemma, we can easily extend our results to stochastic labeling. For instance, Proposition \ref{prop:kjunta_nonbinary} extends to non-deterministic labeling. To see this, note that due to Lemma \ref{lem:pe for stochastic}, equation \eqref{eq:fJ and g_tilde} in the proof of the proposition still holds for stochastic $Y$. The rest of the proof of the proposition only depends on $\fJ$, hence holds for stochastic $Y$. 




==> IntroV10.tex <==
%\noindent{\textbf{Motivation.}}
%In this introductory section, we first motivate our problem which we formulate
%precisely in Section~\ref{sec-formulation}. Then, after reviewing existing literature,
%we present in Section~\ref{sec-summary} a summary of our main results.

%\subsection{Motivation}

Feature selection is critical to the design of learning systems impacting their performance and complexity.
%
%Feature selection is an important learning problem that can be studied under the PAC framework.
In the supervised learning paradigm, studied in this paper, good feature selection can  reduce the training and utilization running time, as well as improve model interpretability \citep{Guyon2003}.  The objective of feature selection can be stated as finding a set of features (say $k$ out of $d$) so that the prediction accuracy remains relatively unchanged. For that, the main challenge is formulating a measure to evaluate the feature subsets. Such a measure needs to be computationally efficient and theoretically justified. Several measures and methods have been introduced in the literature  \citep{Kohavi1997,Koller1996,Battiti1994,Vergara2014,Yu2004,mrmr,Gretton2005,Kernel_feature2017}. However, in general, provable relations between these measures and the prediction accuracy remain open. 
In this work we study the feature selection problem as a \emph{Probably Approximately Correct (PAC)} learning problem.
The PAC framework and its agnostic version were introduced by \citet{Valiant1984} and \citet{Kearns1994}, respectively. Learning under this model has been studied extensively \citep{linial1993constant,Valiant2015,pmlr-v99-goel19b}. 

%The prediction accuracy depends both on the particular learning algorithm as well as the selected features. Hence, makes it harder to analyze the problem.  Therefore, as a first step, one can focus on the effect of the feature selection by employing the best classifier. In this approach, the problem is to evaluate the maximum attainable prediction accuracy as a function of the number of the features and to find the optimal feature subset of the given size.  

We formulate feature selection as an \textit{agnostic PAC} learning problem. The focus of this paper is on supervised binary classification with features taking values on the Boolean hyper-cube.
%\subsection{Problem Formulation}\label{subsec:problem formulation}
%\label{sec-formulation}
%\paragraph{Problem Formulation and Approach}
Our model considers learning mappings from an example, which consists
of $d$ features, to a \emph{binary} label. The mapping should map every 
possible combination of feature values in an example to a label.
In particular, our model observes  $n$ training instances each of which contains $d$ features $\bfx\in \pmm^d$ with labels $y\in \pmm$. The samples are generated \ac{IID}  according to an unknown, but fixed probability distribution $P_{\bfX Y}$. The 0-1 loss function is used to measure the prediction accuracy.  The expectation of this loss over $\P_{\bfX Y}$ is referred to as \textit{misclassification} probability. 
 
 More precisely, in feature selection, given a parameter $k<d$, the objective is to find the set of best $k$ features with a $k$-variable predictor that minimizes the misclassification probability.
 Hence, the set of all $k$-variable predictors $g:\pmm^k\mapsto \pmm$ followed by the selected features $(j_1, j_2, ..., j_k)$ are considered as the target class.  The size of this set is $O(d^k2^{2^k})$ ($O(d^k)$ for selecting a $k$-features combination, and $O(2^{2^k})$ for assigning a dictionary to all possible feature vectors and for all possible dictionaries). The \ac{VC} dimension of the class is between $2^k$ and $2^k+O(k\log d)$ ( \ac{VC} dimension of a hypothesis class is the maximum size of the input set that can be shattered \citep{Shalev2014}). For this target class, the \textit{minimum attainable misclassification probability} is defined as 
 \begin{align*}
\Pek\deq \min_{j_1, j_2, .., j_k\in [d]}~~\min_{g:\pmm^k\mapsto \pmm} \PP_{\bfX,Y}\Big\{Y\neq g(X_{j_1}, X_{j_2},..., X_{j_k})\Big \}.
\end{align*}
 %In this formulation, the coordinates $(j_1, j_2, \cdots, j_k)$ represent the selected features and $g$ represents the $k$-variable predictor.
 In the PAC learning framework, upon observing the training instances, a learning algorithm outputs, with probability $(1-\delta)$, a feature subset of cardinality $k$  with  a predictor so that the resulted misclassification probability is at most $\Pek+\epsilon$, where $\epsilon, \delta \in (0,1)$. The goals are to minimize both, the number of training examples needed to achieve such probabilities, and the complexity of the algorithm.
 
 \subsection{Summary of Our Contributions and Approach} 

In this work, we propose a Fourier-framework to study the feature selection problem.  In our earlier work \citep{Heidari_ISIT19}, we characterized $\Pek$ under the deterministic labeling, i.e., $Y=f(\bfX)$, and under known statistics. \addvj{In this paper, we extend that result to agnostic settings with  stochastic mappings. Further, we propose an agnostic-PAC feature selection and learning algorithm and derive theoretical guarantees for the case where the features are statistically independent.}
\addvj{For the feature selection problem, our algorithm agnostically PAC-learns with sample complexity $O(c_k^2\frac{k^2 2^{2k}}{\epsilon^2}\log \frac{d}{\delta})$ and with $O(nk(2d)^k)$ arithmetic operations (see Theorem \ref{thm:unknownf_and_D}). Table \ref{tab:PAC compare} compares  our approach with well-known PAC learning algorithms adopted to the above feature selection problem.  To the best of our knowledge, both the sample and computational complexities of our algorithm improve upon  previously known PAC-learning algorithms.  In particular, we improve the misclassification probability of  the low-degree algorithm \citep{linial1993constant}, which has a comparable computational complexity. As compared to \citet{Kalai2008}'s approach using $\mathcal{L}_1$-polynomial regression, we obtain a lower sample complexity  and significantly lower computational complexity (especially for large data sets).} These algorithms are explained in Subsection  \ref{subsec:related approaches}. 
%
%If the features are statistically independent, our algorithm agnostically PAC learns with respect to the class of $k$-variable predictors. More precisely, its  misclassification probability is up to $\Pek+\epsilon$ with probability $(1-\delta)$, where $\epsilon, \delta\in (0,1)$. Hence, we can use this algorithm for learning with feature selection and derive theoretical guarantees under the  condition that the features are statistically independent.    The computational complexity of this algorithm is $O(nk(2d)^k)$ and the sample complexity of the algorithm is $O(c_k^2\frac{k^2 2^{2k}}{\epsilon^2}\log \frac{d}{\delta})$, where $c_k$ is a distribution-dependent parameter (see Theorem \ref{thm:unknownf_and_D}). 
%Table \ref{tab:PAC compare} compares  our approach with well-known PAC learning algorithms adopted to the above feature selection problem. These algorithms are explained in Subsection  \ref{subsec:related approaches}. It is observed that our algorithm has the low sample complexity ( close to that of ERM) and with significantly lower computational complexity as compared to other mentioned algorithms. 
Our main contributions are itemized below.




\begin{table}[ht]
\centering
\caption{Comparison of our algorithm with other PAC-learning approaches}
\label{tab:PAC compare}
\begin{tabular}{lccc}
\toprule 
Approach & Sample Cmpx. & Computational Cmpx. & Misclassification Prob. \\ 
\hline \\[-1em]
\begin{minipage}{3.6cm} ERM\\ (Naive Exhaustive)\end{minipage} & { $O(\frac{k2^k}{\epsilon^2}\log\frac{d}{\delta})$}  & $O(nd^k2^{2^k})$ & $\Pek+\epsilon$ \\ [3pt]
\hline \\[-1em]
\begin{minipage}{3.6cm}$\mathcal{L}_1$-Poly. Regression \\ \citep{Kalai2008}\end{minipage} & {$O(d^{\Theta(k)/\epsilon})$} &  $O(n^2d^{(3+\omega)3k})$ & $\Pek+\epsilon$ \\ [3pt]
\hline \\[-1em]
\begin{minipage}{3.6cm} Low-degree Algorithm\\ \citep{linial1993constant} \end{minipage}& $O(2^k \log\frac{1}{\delta})$ & $O(nkd^k)$ & $8\Pek$ (\textit{uniform dist.}) \\ [3pt]
\hline \\[-1em]
Our Approach & $O(c_k^2\frac{k^2 2^{2k}}{\epsilon^2}\log \frac{d}{\delta})$ & $O(nk(2d)^k)$ &  \begin{minipage}{3.6cm} $\Pek+\epsilon$ (\textit{product dist.,  stochastic labeling})\end{minipage} \\ [3pt]
\bottomrule
\end{tabular} 

\end{table}












\paragraph{A Fourier Framework:}
We extend the range of applications of \emph{Fourier expansion on Boolean cubes}, by adapting it to the more general space of stochastic mappings (e.g., mappings from one probability space to another). Then, we develop a framework that allows us to characterize $\Pek$ in the Fourier domain and find the optimal predictor and the feature subset. \addvj{Note that, applying this framework, we do not require any distributional assumption on the label other than taking values from $\pmm$.  }

We leverage
the standard \emph{Fourier expansion on the Boolean cube}, which has been central in a range of other applications such as noise sensitivity \citep{ODonnell2014,kalai2005noise}, and information-theoretic problems \citep{courtade2014boolean}. 
In this expansion, (analogue to standard Fourier series on a periodic function) any real-valued function on the Boolean cube can be expressed as a linear combination of \textit{parities}   \citep{ODonnell2014,Wolf2008}.  The Fourier coefficients quantify the levels of ``nonlinearities'' in a function, and this property can be leveraged to our results.
% Highly nonlinear functions have Fourier expansion with large coefficients for high-degree parities. Thus,  the Fourier expansion is potentially  a powerful tool in the feature selection problem. %However, there are limitations making it impractical for this purpose.  First, it is assumed that the features are mutually independent. Secondly, this expansion is defined only for deterministic functions of the features. 


%Next, we design our algorithm based on this characterization. 

%  Although this Fourier expansion is defined on the Boolean cube, our algorithm is applicable to non-binary features as well. We view the Binary Fourier as a framework that captures a special class of nonlinearities — those characterized via the \textit{parities}.  As a future work, one can adopt the discrete Fourier expansion to non-binary features and, based on it, design the learning algorithms. We believe, such a generalization requires character theory, which is beyond the scope of this paper. We note that there are other forms of orthogonal decomposition including the Hoeffding-Sobel decomposition \citep{HoeffdingDecomp,Sobol1993,Chastaing2012}. However, such decompositions are basis-free. Our Fourier framework is defined by constructing a set of \textit{orthonormal} basis functions which makes it suitable for designing algorithms. 


 
%We, further, propose a second algorithm which is computationally more efficient than our first algorithm. This algorithm is based on estimating a $2$-norm expression as opposed to estimating the $1$-norm quantity in the first algorithm. We show in Theorem \ref{thm:alg2_norm2} that the misclassification probability of the second algorithm is at most $4\Pek$.  We note that the low-degree algorithm is subsumed under our algorithm and its theoretical guarantees \citep{Kalai2008} are extended to agnostic settings with independent features. Also, our results extend that of \citep{Mossel_ODonnell,mossel2004learning} to $k$-junta learning of arbitrary functions with non-uniform input variables.
%
% optimization with sample complexity $O\big( 2^{2k} \frac{1}{\epsilon^2} \log_2(\frac{d^k}{\delta})\big)$ and  running time $O(n 2^k d^k)$, where $n$ is the number of training sample.
%The special case of this problem, where the function $f$ itself depends on only $k$ variables, has been studied in the literature \citep{Mossel_ODonnell,mossel2004learning}. In particular, in \citep{Mossel_ODonnell}, a Fourier based algorithm was introduced for  PAC learning of Boolean $k$-junta functions under the {\it uniform distribution} on the binary features for the features. In our work, $f$ is an arbitrary Boolean function that potentially depends on more than $k$ input variables and the source is general but memoryless.  


\label{sec-summary}
\paragraph{Guaranteed Universal Learning for Independent Features:}
\addvj{
We consider \emph{Universal PAC} learning, i.e., agnostic PAC learning under some distributional (class) restrictions without knowing the actual distribution in the class. From an information-theoretic standpoint, the term \textit{universal} indicates that a data-processing scheme achieves certain theoretical optimalities while agnostic to the statistics of the data \citep{Cover2006}\footnote{Lempel-Ziv \citep{Ziv1977} 
is an example of a universal algorithm. }.   
%The objective of a learning algorithm is to find the ``best" $k$ features and output a predictor with misclassification probability close to the optimal value ($\Pek$). 
That said, we restrict ourselves to agnostic PAC learning under the distributional restrictions that the features are independent. %
%From an information-theoretic standpoint, the objective is to find a learning algorithm for which the misclassification probability converges to $\Pek$ as the number of the samples is growing large (when the statistics of the data are unknown). We call such an algorithm  \textit{universal}\footnote{This terminology is used in lossless data compression \citep{Cover2006}, where the objective is to compress a sequence of samples with the minimum number of bits. Universality implies that the compression algorithm achieves optimality while agnostic to the statistics of the data. Lempel-Ziv \citep{Ziv1977} is an example of such algorithms. } for the class of memoryless sources. This formulation can be viewed as agnostic PAC learning under the distributional restrictions that the features are independent.
We note that, this condition can be relaxed to being almost independent \citep{blais2010polynomial}, that is $P_{\bfX}$ is close to a product probability distribution in \textit{total variation} distance.} %In addition, the independence condition can be further relaxed to satisfying a set of correlation conditions as discussed in \citep{nips20}. }
%More precisely, 
%under such constraints, for any $\epsilon, \delta \in (0,1)$, and 
%sufficiently large number of training samples as a function of $(\epsilon,\delta)$, a universal algorithm should output, 
%with probability at least $(1-\delta)$, a hypothesis  
%with misclassification probability not exceeding $\Pek+\epsilon$, 
%where $f$ is the unknown labeling function. 

\paragraph{Fourier-Based Learning Algorithm:}  
%Next, based on our Fourier framework, we propose an agnostic-PAC learning algorithm. If the features are statistically independent, our algorithm agnostically PAC learns with respect to the class of $k$-variable predictors. That is its the misclassification probability is up to $\Pek+\epsilon$ with probability $(1-\delta)$, where $\epsilon, \delta\in (0,1)$. Hence, we can use this algorithm for learning with feature selection and derive theoretical guarantees under the  condition that the features are statistically independent.  %The significance of our contribution is to adopt a Fourier-based learning algorithm and derive theoretical guarantees under agnostic settings. 
% The computational complexity of this algorithm is $O(nk(2d)^k)$ and the sample complexity of the algorithm is $O(\frac{2^{O(k)}}{\epsilon^2}\log \frac{d}{\delta})$ (see Theorem \ref{thm:unknownf_and_D}). Hence, the algorithm has the low sample complexity ( close to that of ERM) and with significantly lower computational complexity as compared to other mentioned algorithms. 
\addvj{We propose a feature selection algorithm with PAC learning guarantees using lower sample and computations complexities than previously known PAC learning algorithms. %for the same PAC error probability, and better error probability for methods with comparable complexity.
For that, we propose a Fourier-based implementation of $\mathcal{L}_1$ polynomial regression ---  that is an $\mathcal{L}_1$ counterpart of the low-degree algorithm. Hence, our algorithm achieves $\Pek$ with lower computational complexity as compared to $\mathcal{L}_1$ polynomial regression. 
The objective of $\mathcal{L}_1$ polynomial regression is to minimize the \ac{MAE} over all polynomials of a given degree, that is $\min_{p(\bfx)}\EE[|Y-p(\bfX)|]$, where $P(\bfx)$ is a polynomial of fixed degree (say $k$). In $\mathcal{L}_2$ polynomial regression, the objective is to minimize the \ac{MSE}, that is $\min_{p(\bfx)}\EE[(Y-p(\bfX))^2]$.} The low-degree algorithm can be viewed as a computationally more efficient way of implementing $\mathcal{L}_2$ polynomial regression \citep{Kalai2008}. However, due to $\mathcal{L}_2$ polynomial regression, the current PAC learning guarantees are $8\Pek$ in small-error regions. %In this paper, we propose a Fourier-based implementation of $\mathcal{L}_1$ polynomial regression ---  that is an $\mathcal{L}_1$ counterpart of the low-degree algorithm. Further, we extend this algorithm to agnostic learning under unknown product probability distributions. 
We address this issue by implementing $\mathcal{L}_1$ regression instead of $\mathcal{L}_2$. Hence, benefiting  from the learning capability of $\mathcal{L}_1$ regression as well as computational efficiency of the low-degree algorithm.
%as a Fourier-based approach is computationally more efficient as compared to $\mathcal{L}_1$ polynomial regression. In fact, it can be viewed as a computationally more efficient way of implementing $\mathcal{L}_2$ polynomial regression \citep{Kalai2008}. However, there are two issues restricting the applications of this approach: 1) due to $\mathcal{L}_2$ polynomial regression, the current guarantees are $8\Pek$ in small-error regions. 2) The features' distribution is assumed to be known and uniform.

%We address the first issue by implementing a $\mathcal{L}_1$ polynomial regression with a Fourier-based algorithm ---  that is a $\mathcal{L}_1$ counterpart of the low-degree algorithm. We address the second issue, by extending the Fourier framework to product probability spaces and to stochastic mappings. 



 Via a large deviation analysis based on Azuma's inequality for the concentration of martingales \citep{Azuma1967,Szpankowski2011}, we provide bounds on the rate of the convergence of the algorithm's misclassification probability. More precisely, we show in Theorem \ref{thm:regret} that the expected misclassification probability of the algorithm converges to $\Pek$ with rate  $O(n^{-\gamma})$ for some $\gamma<1/2$.

\paragraph{Other Applications.}
Building upon the prior concentration results \citep{blais2010polynomial}, our algorithm can be used in other fundamental problems in computational learning, such as \textit{agnostic} PAC learning with respect to \textit{linear threshold} functions and the class of $\alpha(\epsilon,k)$ concentrated functions, that is a collection of functions each of which approximated by a polynomial of degree $k$ with \ac{MSE} at most $\epsilon$.   Also, our Fourier-based measure can be used in feature selection problems to evaluate the feature subsets. One can adopt conventional search algorithms ( e.g., the greedy algorithm or ranking methods) with our measure for feature selection. 


%We can show that our results hold when the features are ``almost" independent, that is $P_{\bfX}$ is close to a product probability distribution in \textit{total variation} distance. %We further can adapt our analysis to arbitrarily dependent features \citep{nips20}. %Further, our results extend to learning problems in which the features, although dependent, form groups of ``almost" independent super-features.
 
 
 
 
 
 
 
 
 
 
 
 
 \subsection{Related Approaches} \label{subsec:related approaches}
Several approaches have been proposed in the literature for the feature selection problem with PAC guarantees.  We briefly review them below. %In what follows, we present an overview of a few existing methods. 

\paragraph{Naive  \ac{ERM}:}
This is an exhaustive search over all feature subsets and predictors to minimize the empirical misclassification rate. For our problem, ERM is a PAC learning algorithm with  sample complexity of $O(\frac{k2^k}{\epsilon^2}\log\frac{d}{\delta})$ and with computational complexity $O(nd^k2^{2^k})$ \citep{Shalev2014}. With the computational complexity of doubly exponential with respect to $k$, ERM is prohibitive even for small values of $k$.

\paragraph{$\mathcal{L}_1$ Polynomial Regression and SVM.}
  \citet{Kalai2008} introduced polynomial regression as an approach for PAC learning with the $0-1$ loss function. They showed that $\mathcal{L}_1$-Polynomial regression agnostically PAC learns with respect to a $(k,\epsilon)$-concentrated hypothesis class. Recently, \citet{blais2010polynomial} provided some generalizations of this class. 
Adopting this algorithm to our problem, with an exhaustive search over feature subsets, requires a sample complexity $O(d^{\Theta(k)/\epsilon})$. With a \textit{linear programming} implementation, the computational complexity of this algorithm is $O(n^2d^{(3+\omega)3k})$, where $\omega < 2.4$ is the matrix-multiplication exponent. A more efficient implementation is \ac{SVM} with degree-$k$ polynomial kernel and without any regularization \citep{Kalai2008}. This implementation PAC learns in the non-agnostic setting, that is when the target labeling function itself belongs to the hypothesis class. However, this is not the case in the agnostic setting and when $\Pek$ is away from zero \citep{blais2010polynomial}. 
% Kalai, et al. showed that $L_1$ polynomial regression agnostically PAC learn with respect to the class of \textit{threshold functions} under the uniform distribution. The authors in \citep{blais2010polynomial} extended this result to  \textit{mixtures} of arbitrary product probability distributions. %Despite these promising results, due to its computational complexity, polynomial regression is prohibited in practical applications. 


\paragraph{Low Degree Algorithm.}
\citet{linial1993constant} investigated PAC learning from an alternative perspective under a distributional restriction on $\bfX$ and introduced the well-known ``Low-Degree Algorithm". They provide  theoretical guarantees  under the {\it uniform} and {\it known} distribution on $\pmm^d$ of the examples. As \citet{Kalai2008} showed, under the uniform distribution, the low-degree algorithm agnostically learns the $(k,\epsilon)$-concentrated hypothesis classes with an error up to $8\Pek+\epsilon$. This algorithm is based on the Fourier expansion on the Boolean hyper-cube. Although  computationally efficient, this algorithm has limited practical applications due to its distributional restrictions --- uniform (and known) distribution is unrealistic in many applications.  Further, the factor $8$ in the accuracy bound is noticeable when $\Pek$ is not close to zero (say $\approx 0.1$). \citet{furst1991improved} relaxed such a distributional restriction by adopting a low-degree algorithm for learning $AC^0$ functions under the product probability distributions. However, the second issue (factor $8$) remains to be resolved.  %However, there are two issues restricting the applications of this approach: 1) due to $\mathcal{L}_2$ polynomial regression, the current guarantees are $8\Pek$ in small-error regions. 2) The features' distribution is assumed to be known and uniform.

\addvj{
The Fourier estimation approach in the low-degree algorithm has interesting properties which makes it suitable for other applications \citep{Mossel_ODonnell,mossel2004learning,Jackson1997}. Such works, mainly, consider PAC learning in \emph{non-agnostic} setting (in which the error probability is zero or sufficiently close to zero) and the under uniform distribution. In this paper, we extend the applications of Fourier estimation to \emph{agnostic} setting involving stochastic mappings. Therefore, we significantly relax the distributional assumptions about the features as well as the target labeling.  Also, we provide a rigorous theoretical analysis guaranteeing the PAC learning capabilities of our algorithm (see Theorem~\ref{thm:unknownf_and_D} and \ref{thm:regret}). }
% makes our approach suitable for more practical 
%In particular,  \citet{Mossel_ODonnell} introduced a Fourier based algorithm for  PAC learning Boolean $k$-junta functions under the {\it uniform distribution}. In this paper, we build upon the Fourier expansion and propose a learning algorithm which has significantly more relaxed distributional assumptions. Further, we show that our algorithm agnostically PAC learns with high accuracy.



 %A special case of this problem, where the target function $f$ itself depends on only $k$ variables, has been studied in the literature \citep{Mossel_ODonnell,mossel2004learning}.  on the binary features for the features. 
%In our work, $f$ is an arbitrary Boolean function that potentially depends on more than $k$ input variables and the source is general but memoryless. Under these conditions, the low degree algorithm PAC learns when the labeling function is itself a $k$-junta. In \citep{Mossel_ODonnell}, proposed a more efficient Fourier based algorithm for PAC learning of Boolean $k$-junta functions under the uniform distribution. 

 
%The Fourier expansion has been  used to analyze Boolean functions  in wide range of applications, e.g., to characterize the learning complexity \citep{linial1993constant,mossel2004learning}, noise sensitivity \citep{ODonnell2014,kalai2005noise,LiMedardISIT18}, approximation \citep{blais2010polynomial}, and other information-theoretic properties \citep{courtade2014boolean,weinberger2017optimal,weinberger2018self}.  $p$-biased Fourier analysis was used in \citep{furst1991improved}  to show that a certain class of Boolean functions could be learned efficiently using examples drawn from a biased input distribution. It has also been used to study the threshold phenomena of random graphs \citep{talagrand1994russo}.


 



%The focus of this work, from computational theory perspective, is agnostic PAC learning with respect to the class of $k$-junta functions under the arbitrary product probability distribution.
%
% We propose a Fourier-based algorithm that agnostically learns with respect to $k$-juntas.    

 











% We build upon the results in the previous cases and design two learning algorithms. We prove that the prediction accuracy of these algorithms converges to the optimality (i.e., $\Pek$ as in \equationref{eq:k-junta appx}) under two conditions: 1) the features are ``almost" independent, and  2) the features are not trivial random variables. The first algorithm is a plug-in approach and the idea is to estimate the expectation of each feature and plug it in the learning algorithm designed for known distribution. The sample complexity of this algorithm is at most $2^k~ poly(2^{k},\log d)$. The second algorithm is a direct approach with sample complexity  $poly(\frac{1}{p_{\min}^{2k}}, \log d)$, where $p_{\min}$ is the minimum bias among the features.
%



%In more general settings, suppose that  most of the features are  independent, except a group of them which are statistically dependent. In such cases, one can group the dependent features into a  super-feature with a larger value-set. Therefore, as we consider non-binary features, our results extends to learning problems in which the features, although dependent, form groups of ``almost" independent super-features.  
%As a future work, we plan to extend our results to correlated features by adopting more general decomposition techniques such as Hoeffding-Sobol Decomposition \citep{Hooker2007,Champion2013}.       

%\paragraph{Fourier-Based Measure for Feature Selection.} We use a Fourier analysis to propose a new measure for evaluating feature subsets. %Further, we introduce a novel Fourier-based learning algorithm with a class of embedded feature selection methods based on the proposed measure. The embedded feature selection and learning design are such that the computations in one (feature selection) are recycled in the other (the learning algorithm).  Under certain assumptions,  we provide a theoretical justification for the feature selection measure and analyze the performance of the learning algorithm. 
%We show that, given a feature subset $\mathcal{J}$, this measure is equivalent to the misclassification probability of the Bayes learner restricted to $\mathcal{J}$. %Thus, this measure estimates the best attainable accuracy rate when a particular feature subset is used. 
%This is a more accurate estimation comparing to mutual information that only gives bound on the misclassification of the Bay's learner \citep{FederMerhav1994}. Based on this measure and inspired by the approach in \citep{Mossel_ODonnell}, we propose a learning algorithm with an embedded feature selection. 

%For practical applications, one can adopt conventional search algorithms ( e.g., the greedy algorithm or ranking methods) with our measure for feature selection.  Once a feature subset is selected,  our method can be used to construct the predictor. 
%In this approach, there is no theoretical guarantee that the selected features are optimal. But, 
% given the selected feature subset,  the accuracy rate of the predictor converges to that of the Bayes' learner applied to these features.

 %Suppose a search algorithm queries the score of $m$ feature subsets, where each contains at most $k$ features. Then, we show that our measure is close to the Bayes 
%misclassification probability for all the $m$ feature subsets, if there are 
%at least $2^{O(k)} O(\log m)$ number of training samples 
% On one extreme, the exhaustive search can be used in the algorithm to find the best $k$ feature according to the proposed measure. The running time of this feature selection is $O(n 2^k d^k)$. In this case, the computations in the feature selection method are used in the learning and hence the running time of the learning part is negligible. We show that the accuracy rate of the learning algorithm converges to optimality under the condition that features are statistically ``almost" independent. % From an information-theoretic perspective, the propped algorithm is universally optimal under the almost-independent condition --- it achieves optimality while the features' distribution is unknown to the learning algorithm. 
% On the other extreme, where there are tight restrictions on the computational complexity, 
%the feature ranking method can be employed in our algorithm. The running time of 
%this feature selection is $O(nkd)$ and the running time of the learning algorithm is $O(nk2^k)$.
% For a given selected feature subset, in this case, we can prove that 
%the accuracy rate of the algorithm converges to the optimal miscalculation probability 
%(i.e., Bayes' learner applied 
%to the selected features).  However, in this case, there is no theoretical 
%guarantee that the selected features are optimal. 
%As another approach, one 
%can employ conventional search algorithms such as the greedy algorithm with 
%the forward or backward search. For these cases, we provide a sample complexity analysis. 
%%SPA: Maybe the rest can go?
%Suppose a search algorithm queries the score of $m$ feature subsets, where each contains 
%at most $k$ features. Then, we show that our measure is close to the Bayes 
%misclassification probability for all the $m$ feature subsets, if there are 
%at least $2^{O(k)} O(\log m)$ number of training samples.
%
%%\paragraph{Almost Memoryless {\color{red} (To be completed)}} Our analysis works in almost independent features. 

%\subsection{Approach}
%\paragraph{$k$-Junta Approximation} .... As a naive strategy, one could employ an exhaustive search over all $k$-juntas to find the optimal approximation of $f$. In this case, the search space grows at least doubly exponential with $k$ \footnote{The number of all $k$-juntas is between $2^{|\pmm|^k}$ to $O(d^k)2^{|\pmm|^k}$.}. In our earlier work \citep{Heidari_ISIT19}, we characterized the minimum attainable misclassification probability and the optimal $k$-junta approximation of $f$. For that, we adopt the Fourier analysis developed for functions of random variables \citep{ODonnell2014}. As a result of our characterization, the size of the search space is reduced to $O(d^k)$. The main idea is to rewrite the above optimization problem in the Fourier domain and characterize the optimal solution in terms of the Fourier coefficients. Then, based on the Fourier coefficients, the optimal $k$-junta approximation is characterized. 

%\paragraph{Features with Known First and Second Moments}
%As a next step, building upon these theoretical understandings, we study a less ideal case where only a certain number of training instances are available. The training instances are generated according to a \textit{known} distribution which is assumed to be close, in total variation distance, to a product of probability distributions $\prod_{i=1}^d P_{X_i}$. The special case of this problem, where the function $f$ itself depends on only $k$ variables, has been studied in the literature \citep{Mossel_ODonnell,mossel2004learning,blais2010polynomial,goel19b}. In this work, $f$ is an arbitrary Boolean function that potentially depends on more than $k$ input variables.  Inspired by the approach in \citep{Mossel_ODonnell}, we design a  Fourier-based learning algorithm.  The main idea behind this algorithm is to use the training samples to approximate the Fourier coefficients of $f$ with sufficient accuracy. Then, based on our results in the ideal case, we construct a $k$-junta approximation of $f$. We provide the rate of convergence of the algorithm as a function of the number of training samples. For that, we adopt a large deviation analysis based on Azuma's inequality \citep{Szpankowski2011}. The sample complexity of the algorithm is $poly(2^k,\log d)$.


%\paragraph{Universal Learning}
%Next, we study the non-ideal case where the labeling function and the distribution on the features are unknown. We build upon the results in the previous cases and design two learning algorithms. We prove that the prediction accuracy of these algorithms converges to the optimality (i.e., $\Pek$ as in \equationref{eq:k-junta appx}) under two conditions: 1) the features are ``almost" independent, and  2) the features are not trivial random variables. The first algorithm is a plug-in approach and the idea is to estimate the expectation of each feature and plug it in the learning algorithm designed for known distribution. The sample complexity of this algorithm is at most $2^k~ poly(2^{k},\log d)$. The second algorithm is a direct approach with sample complexity  $poly(\frac{1}{p_{\min}^{2k}}, \log d)$, where $p_{\min}$ is the minimum bias among the features.


 

%\paragraph{Justify the memoryless assumption.}
%Theoretical guarantees can be extended to the case where the features are almost independent. But for the general case, the guarantees will vanish, but one can still use the algorithms. In these cases, one can combine the correlated features to make a hybrid one. 
%Extension to almost memoryless
%\subsection{Related Works}




==> Proof_lemma_festS.tex <==
Note that if $\mathcal{T}\subseteq \mathcal{S}$
\begin{align*}
\<\psi_\mathcal{T}, \pestS\>= \prod_{j\in \mathcal{T}}(\frac{\sigma_j}{\bar{\sigma}_j})\prod_{l\in \mathcal{S}/\mathcal{T}}(\frac{|\mu_l-\bar{\mu}_l|}{\bar{\sigma}_l})
\end{align*}
otherwise $\<\psi_\mathcal{T}, \pestS\>=0$. For any subset $\mathcal{A}\subseteq [d]$, define $b_{\mathcal{A}}\deq \prod_{j\in \mathcal{A}}(\frac{\sigma_j}{\bar{\sigma}_j})$ and $d_{\mathcal{A}}\deq \prod_{l\in S/T}(\frac{|\mu_l-\bar{\mu}_l|}{\bar{\sigma}_l})$.  As a result, the $p$-biased Fourier expansion of $\pestS$ is given by 
\begin{align}\label{eq:Fourier_phi bar}
\pestS(x^d)= \sum_{\mathcal{T}\subseteq \mathcal{S}} b_\mathcal{T}~d_{\mathcal{S}/\mathcal{T}} ~\psi_\mathcal{T}(x^d)
 \end{align} 
From this Fourier expansion and Parseval's inequality we have that
 \begin{align*}
 \norm{\festS ~\pestS - \fbarS~ {\psi}_S  }_2^2 &=\big(\fbarS- b_\mathcal{S}~\festS\big)^2+ \festS^2  \sum_{T\subset S} b_\mathcal{T}^2~d_{\mathcal{S/T}}^2\\
 &\stackrel{(a)}{=}\big(\fbarS- b_\mathcal{S}~\festS\big)^2 +\festS^2\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)-\festS^2 b_\mathcal{S}^2\\
 &=\fbarS^2- 2 b_\mathcal{S}~\fbarS \festS +\festS^2\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)\\  \numberthis \label{eq:fest_phibarS 1}
 &=\fbarS\Big[ \fbarS- b_\mathcal{S}~ \festS\Big] + \festS \Big[ \festS~\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)-\fbarS\Big]  
  \end{align*} 
 where $(a)$ follows from the identity  $$\sum_{\mathcal{T}\subseteq \mathcal{S} } \prod_{j\in \mathcal{T}}a_j \prod_{l\in \mathcal{S/T}}b_l=\prod_{j\in \mathcal{S}}(a_j+b_j).$$ By the definition of $b_{\mathcal{S}}$, the first term in \meqref{eq:fest_phibarS 1} is upper bounded as
 \begin{align*}
\fbarS\Big[ \fbarS- b_{\mathcal{S}}~ \festS\Big] &\stackrel{(a)}{\leq} | \fbarS| ~|1- b_{\mathcal{S}}| + b_{\mathcal{S}} ~\big| \fbarS- \festS\big|\\
&\stackrel{(b)}{\leq}  |1- b_{\mathcal{S}}| + b_{\mathcal{S}} ~\big| \fbarS- \festS\big|\\
&\stackrel{(c)}{\leq} |1- b_{\mathcal{S}}| +(1+\epsilon)^{|\mathcal{S}|}~\big| \fbarS- \festS\big|\\
&\stackrel{(d)}{\leq}(e^{k\epsilon}-1)+e^{k\epsilon} ~\big| \fbarS- \festS\big|
 \end{align*}
 where $(a)$ follows by the triangle inequality and adding and subtracting  $b_{\mathcal{S}}~ \fbarS$. Inequality $(b)$ is because $ \fbarS \leq 1$, and $(c)$ follows because, from the lemma's assumptions, $b_{\mathcal{S}}\leq (1+\epsilon)^{|\mathcal{S}|}$. Lastly, inequality $(d)$ is because of the following argument. From the assumption of the lemma we obtain that
 \begin{align*}
 1-(1+\epsilon)^{|S|}\leq            1- b_{\mathcal{S}}\leq  1-(1-\epsilon)^{|S|}.
 \end{align*}
 Since $\epsilon \in (0,1)$ and $|S|\leq k$, then $(1-\epsilon)^{|S|}\geq 1-k\epsilon $. Also, from the fact that $(1+x)\leq e^x$ for all $x\in \RR$, we obtain
  \begin{align}\label{eq:bound on c_S}
1-e^{k\epsilon}\leq  1- b_{\mathcal{S}}\leq  k\epsilon \leq e^{k\epsilon}-1.
 \end{align}
Lastly, applying from the inequality   $(1+\epsilon)^k\leq e^{k\epsilon}$ completes the proof of inequality $(d)$.
% \begin{align*}
% \fbarS\Big[ \fbarS- (\frac{\sigma}{\bar{\sigma}})^{|S|}~ \festS\Big]\leq (e^{k\epsilon}-1)+e^{k\epsilon} ~\big| \fbarS- \festS\big|
% \end{align*}

As for the second term in \meqref{eq:fest_phibarS 1}, by adding and subtracting $\fbarS~\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)$, we have  
 \begin{align}\label{eq:secondterm_festS}
 \festS  \Big[ \festS~\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)-\fbarS\Big]\leq \Big| 1-\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)\Big|+ \prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)\big|\festS -\fbarS\big|
 \end{align}
From the assumptions in the lemma   $b_{\{j\}} \in (1\pm \epsilon)$ and $d_{\{j\}}\in (0, \frac{\epsilon}{\bar{\sigma}_j})$. Therefore, from the inequality $\sigma_j\leq \bar{\sigma}_j (1+\epsilon)$, we get that
 \begin{align*}
1+\epsilon^2-2\epsilon \leq  (b_{\{j\}}^2+d_{\{j\}}^2)\leq 1+\epsilon^2+2\epsilon+\frac{\epsilon(1+\epsilon)}{{\sigma}_j}
 \end{align*}
 which implies 
 \begin{align*}
-(3\epsilon+\frac{\epsilon(1+\epsilon)}{{\sigma}_j})\leq (b_{\{j\}}^2+d_{\{j\}}^2) -1 \leq 3\epsilon+\frac{\epsilon(1+\epsilon)}{{\sigma}_j}
 \end{align*}
 Therefore, as $\sigma_{\min}\leq \sigma_j$ for all $j\in \mathcal{S}$, we have
 \begin{align}\label{eq:b_j^2+d_j^2}
\Big| 1-\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)\Big|\leq e^{k\epsilon(3+\frac{1+\epsilon}{{\sigma}_{\min}})}-1
 \end{align}
 Hence, the right-hand side of \eqref{eq:secondterm_festS} does not exceed 
 \begin{align*}
 (e^{k\epsilon(3+\frac{1+\epsilon}{{\sigma}_{\min}})}-1)+e^{k\epsilon(3+\frac{1+\epsilon}{{\sigma}_{\min}})}~ \big|\festS -\fbarS\big|
 \end{align*}
 This is an upper bound on the second term in  \meqref{eq:fest_phibarS 1}. Combining this bound with the one on the first term in  \meqref{eq:fest_phibarS 1} completes the proof. 
%\begin{align*}
%\norm{\festS ~\bar{\phi}_S - \fbarS~ {\phi}_S  }_2^2 &\leq (e^{k\epsilon}-1)+e^{k\epsilon}~\big| \fbarS- \festS\big| + (e^{k(3\epsilon+\frac{\epsilon}{\bar{\sigma}})}-1)+e^{k(3\epsilon+\frac{\epsilon}{\bar{\sigma}})}~ \big|\festS -\fbarS\big|\\
%&\leq 2(e^{k(3\epsilon+\frac{\epsilon}{\bar{\sigma}})}-1)+2e^{k(3\epsilon+\frac{\epsilon}{\bar{\sigma}})}~ \big|\festS -\fbarS\big|
%\end{align*}




==> Proof_lemma_mubar.tex <==
%\section{Proof of Lemma \ref{lem:mean_est}}\label{appx:mean_est}
From triangle inequality
\begin{align*}
|\festS-\fbarS|\leq \frac{1}{n}\sum_{i}|\pestS(\mathbf{x}(i))-\pS(\mathbf{x}(i))|\leq \norm{\pS-\pestS}_{\infty}
\end{align*}
%Let $\Delta_S^{(n)}\deq \frac{1}{n}\sum_{i}|\pestS(\mathbf{x}(i))-\pS(\mathbf{x}(i))|$. We apply Azuma's inequality to prove that with high probability $\Delta_S^{(n)}$ is sufficiently small. For this purpose, we need to find the constants $c_i$ as in Lemma \ref{lem:Azuma}. That said, we find functions $\nu(\epsilon')$ and $\gamma(\epsilon')$ such that 
%\begin{align*}
%\EE[\Delta_S^{(n)}]\leq \nu(\epsilon'), \qquad c_i\leq \gamma(\epsilon')
%\end{align*}
%As the training samples are drawn independently, $c_i=\norm{\pS-\pestS}_{\infty}$. Further, 
%\begin{align*}
%\EE[\Delta_S^{(n)}]\leq   \EE_{X^d}|\pestS(X^d)-\pS(X^d)|=\norm{\pestS-\pS}_1
%\end{align*}
The proof is complete by the following Lemma:
\begin{lem}
Given $\epsilon'\in (0,1)$ suppose $|\bar{\mu}_j-\mu_j|\leq \epsilon'$ and $|1-\frac{\sigma_j}{\bar{\sigma}_j}|\leq \epsilon'$ for all $j\in [d]$. Then, almost surely, $\norm{\pS-\pestS}_{\infty}\leq \gamma(\epsilon')$, where $\gamma(\epsilon')=k  \epsilon' (1+\frac{1}{\sigma_{\min}}e^{2k\epsilon'})\sqrt{c_k}$.
\end{lem}
\begin{proof}
 We start with the triangle inequality for $\infty$- norm.
\begin{align*}
\norm{\pS-\pestS}_{\infty}&\leq \norm{\pS-b_{\mathcal{S}}\pS}_{\infty}+\norm{b_{\mathcal{S}}\pS-\pestS}_{\infty}\\
&=(1-b_{\mathcal{S}})\norm{\pS}_{\infty}+   \norm{b_{\mathcal{S}}\pS  \pm  \big(\sum_{l\in \mathcal{S}}  \prod_{i\leq l} \frac{x_i-\bar{\mu}_i}{\bar{\sigma}_i} \prod_{r> l} \frac{x_r-\mu_r}{\bar{\sigma}_r}  \big)-\pestS}_{\infty} \\
&\leq k\epsilon'\norm{\pS}_{\infty}+ \prod_{j\in S} \frac{1}{\bar{\sigma}_j} \sum_{l\in \mathcal{S}} |\mu_l-\bar{\mu}_l|~  \norm{\prod_{i< l} (x_i-\bar{\mu}_i) \prod_{r> l} (x_r-\mu_r)}_{\infty}\\
&\leq k\epsilon' \norm{\pS}_{\infty}+\frac{k\epsilon'}{\sigma_{\min}} b_{\mathcal{S}}  (1+\epsilon')^k\norm{\pS}_{\infty}\\
&\leq  k\epsilon' \norm{\pS}_{\infty}+\frac{k\epsilon'}{\sigma_{\min}} (1+\epsilon')^{2k}\norm{\pS}_{\infty}\\
&\leq  k\epsilon' \norm{\pS}_{\infty}  \big(1 +\frac{1}{\sigma_{\min}} e^{2k}\big)
 \end{align*} 
 The proof is complete by noting that $\norm{\pS}_{\infty} \leq \sqrt{c_k}$.
\end{proof}




\begin{comment}
\begin{lem}\label{lem:phi_phihat}
Given $\epsilon'\in (0,1)$ suppose $|\bar{\mu}_j-\mu_j|\leq \epsilon'$ and $|1-\frac{\sigma_j}{\bar{\sigma}_j}|\leq \epsilon'$ for all $j\in [d]$. Then, for any subset $\mathcal{S}\subset [d]$ with at most $k$ elements, the following inequalities hold
\begin{align*}
\norm{\pS-\pestS}_1&\leq \nu(\epsilon'), \qquad \norm{\pS-\pestS}_{\infty}\leq \gamma(\epsilon')
\end{align*}
where 
\begin{align*}
\nu(\epsilon')&=k\epsilon'\big(1+(3+\frac{1+\epsilon'}{{\sigma}_{\min}})e^{k\epsilon'(3+\frac{1+\epsilon'}{{\sigma}_{\min}})}\big)\\
\gamma(\epsilon')&=k  \epsilon' (1+\frac{1}{\sigma_{\min}})e^{2k\epsilon'}\sqrt{c_k}
\end{align*}


\end{lem}
\begin{proof}
From the identity $\norm{}_1\leq \norm{}_2$, it suffices to bound the $2$-norm. Hence, from the definition of  $2$-norm, we have 
\begin{align*}
\norm{\pS-\pestS}_2^2&=\norm{\pS}_2^2+\norm{\pestS}_2^2-2\EE[ \ps(X^d) \pestS(X^d)]\\
&\stackrel{(a)}{=}1+\prod_{j\in \mathcal{S}} \EE\Big[\frac{(X_j-\bar{\mu}_j)^2}{\bar{\sigma}^2_j}\Big]-2 \prod_{j\in \mathcal{S}} \EE\Big[\frac{(X_j-\bar{\mu}_j)(X_j-\mu_j)}{\sigma_j \bar{\sigma}_j}\Big]\\
&\stackrel{(b)}{=}1+\prod_{j\in \mathcal{S}}(b_{\{j\}}^2+d_{\{j\}}^2)-2b_{\mathcal{S}}\\
&\stackrel{(c)}{\leq} 1+e^{k\epsilon'(3+\frac{1+\epsilon'}{{\sigma}_{\min}})}-2(1-k\epsilon')\\
&\leq e^{k\epsilon'(3+\frac{1+\epsilon'}{{\sigma}_{\min}})}-1 + k\epsilon'\\
&\leq k\epsilon'\big(1+(3+\frac{1+\epsilon'}{{\sigma}_{\min}})e^{k\epsilon'(3+\frac{1+\epsilon'}{{\sigma}_{\min}})}\big),
\end{align*}
where $(a)$ follows as $X_j$'s are uncorrelated, $(b)$ is due to the definition of  $b_{\{j\}}, d_{\{j\}}$ and $b_{\mathcal{S}}$, and  $(c)$ follows from \meqref{eq:bound on c_S} and \eqref{eq:c_j^2+d_j^2}. 

Next, we prove the second inequality in the lemma. We start by defining the subsets $\mathcal{S}_{ > i}\deq \{j\in \mathcal{S}: j>i\}$ and $\mathcal{S}_{ < i}\deq \{j\in \mathcal{S}: j<i\}$.  We start with the triangle inequality for $\infty$- norm.
\begin{align*}
\norm{\pS-\pestS}_{\infty}&\leq \norm{\pS-b_{\mathcal{S}}\pS}_{\infty}+\norm{b_{\mathcal{S}}\pS-\pestS}_{\infty}\\
&=(1-b_{\mathcal{S}})\norm{\pS}_{\infty}+   \norm{b_{\mathcal{S}}\pS  \pm  \big(\sum_{l\in \mathcal{S}}  \prod_{i\leq l} \frac{x_i-\bar{\mu}_i}{\bar{\sigma}_i} \prod_{r> l} \frac{x_r-\mu_r}{\bar{\sigma}_r}  \big)-\pestS}_{\infty} \\
&\leq k\epsilon'\norm{\pS}_{\infty}+ \prod_{j\in S} \frac{1}{\bar{\sigma}_j} \sum_{l\in \mathcal{S}} |\mu_l-\bar{\mu}_l|~  \norm{\prod_{i< l} (x_i-\bar{\mu}_i) \prod_{r> l} (x_r-\mu_r)}_{\infty}\\
&\leq k\epsilon' \norm{\pS}_{\infty}+\frac{k\epsilon'}{\sigma_{\min}} b_{\mathcal{S}}  (1+\epsilon')^k\norm{\pS}_{\infty}\\
&\leq  k\epsilon' \norm{\pS}_{\infty}+\frac{k\epsilon'}{\sigma_{\min}} (1+\epsilon')^{2k}\norm{\pS}_{\infty}
 \end{align*} 
\end{proof}





Next, we apply Azuma's inequality.
\begin{align*}
\prob{| \Delta_S^{(n)}- \EE[ \Delta_S^{(n)}]|\geq \epsilon'' }\leq 2\exp\left\{-n \frac{\epsilon''^2}{2\gamma(\epsilon')^2}   \right \}
\end{align*}
Note that the event $| \Delta_S^{(n)}- \EE[ \Delta_S^{(n)}]|\geq \epsilon''$ implies that 
\begin{align*}
|\festS-\fbarS|=\Delta_S^{(n)}\leq \EE[ \Delta_S^{(n)}] +\epsilon''\geq \nu(\epsilon')-\epsilon''.
\end{align*}
Thus, setting $\epsilon''=\frac{1}{2}\nu(\epsilon')$ and applying the union bound give
\begin{align*}
\PP\Big\{\bigcup_{\mathcal{S}\subseteq [d], |\mathcal{S}|\leq k}\big\{ |\festS-\fbarS| \geq \frac{1}{2}\nu(\epsilon') \big\}~ \Big\}&\leq kd^k\exp\left\{-n \frac{\nu(\epsilon')^2}{8\gamma(\epsilon')^2}   \right \}
\end{align*}

As a result, the above probability is guaranteed to be less than $\delta'$, if 
\begin{align*}
n&\geq  8 (\frac{\gamma(\epsilon)}{\nu(\epsilon')})^2 \log(\frac{kd^k}{\delta'})
\end{align*}
 It is not difficult to show that $\frac{\gamma(\epsilon)}{\nu(\epsilon')}\leq\frac{\sqrt{c_k}}{2}  e^{-k\epsilon'(1+\frac{1+\epsilon'}{{\sigma}_{\min}})}$. Thus, it is sufficient to have 
 \begin{align*}
n&\geq   2 c_k e^{-2k\epsilon'(1+\frac{1+\epsilon'}{{\sigma}_{\min}})}\log(\frac{kd^k}{\delta'})
\end{align*}

\end{comment}
%\end{proof}

%\begin{align*}
%\PP\Big\{\mathcal{E}(\epsilon')\bigcap_{S\subseteq [d], |S|\leq k}\big\{ \Delta_S^{(N-M)}\leq \epsilon \big\}~ \Big\}&=\PP\big\{\mathcal{E}(\epsilon') \big\}\PP\Big\{\bigcup_{S\subseteq [d], |S|\leq k}\big\{ \Delta_S^{(N-M)}\geq \epsilon \big\}~ \big|~ \mathcal{E}(\epsilon') \Big\}\\
%&\geq (1-\delta_0)(1-\delta_1)  
%\end{align*}




%
%\begin{align*}
%\tilde{\mu}&=\frac{1}{nM}\sum_{i=1}^{M}\sum_{j=1}^n x_j(i)\\
%\bar{\mu}&=\max\big\{-(1-\varepsilon_0), \min\{\tilde{\mu}, 1-\varepsilon_0 \}\big\}
%\end{align*}




%\begin{claim}
%Suppose $|\mu|\neq 1$, $|\bar{\mu}-\mu|\leq \epsilon'$. Then
%\begin{align*}
%\big|\frac{\bar{\sigma}}{\sigma}-1\big|&\leq \frac{\epsilon'}{\sigma \min\{\sigma, \bar{\sigma}\}}
%\end{align*}
%\end{claim}
%\begin{proof}
%Assuming that $|\mu|<1$, from Taylor's theorem, for any $\bar{\mu}\in (1\pm\epsilon_0)$, there exists $\xi$ between $\mu$ and $\bar{\mu}$ such that  
%\begin{align*}
%\bar{\sigma}=\sigma-\frac{\xi}{\sqrt{1-\xi^2}}(\bar{\mu}-\mu)
%\end{align*}
%As a result, since $|\xi|\leq \max\{ |\mu|, |\bar{\mu}|\}\leq 1$ then 
%\begin{align*}
%\big|\frac{\bar{\sigma}}{\sigma}-1\big|&=|\frac{\xi}{\sqrt{1-\xi^2}}(\bar{\mu}-\mu)|\\
%&\leq \frac{1}{\min\{\sigma, \bar{\sigma}\}}\frac{|\bar{\mu}-\mu|}{\sigma}\\
%&\leq \frac{\epsilon'}{\sigma \min\{\sigma, \bar{\sigma}\}}
%\end{align*}
%\end{proof}


%\begin{claim}
%Suppose $|\mu|\neq 1$, $|\bar{\mu}-\mu|\leq \epsilon'$. Then
%\begin{align*}
%\norm{\pestS-\pS}_1&\leq k \frac{\epsilon'}{\bar{\sigma}^2} e^{k\frac{\epsilon'}{\bar{\sigma}^2}}, \quad \text{for all subsets }~ S, \text{with}~|S|\leq k.
%\end{align*}
%\end{claim}



==> draft_lin_threshold.tex <==
\begin{theorem}
For any $\epsilon >0$ 
\begin{align*}
\Pek \geq \frac{1}{2} - \frac{ 1}{2}\norm{\Pi_Y^{\epsilon}}_1 - \epsilon,
\end{align*}
where $\Pi_Y^{\epsilon}$ is a polynomial of degree upto $O(\frac{\sqrt{d}}{\epsilon}\log\frac{1}{\epsilon})$ minimizing  
\begin{align*}
\Pi_Y^{\epsilon} \deq \argmin_{p: \degree < O(\frac{\sqrt{d}}{\epsilon}\log\frac{1}{\epsilon})} \norm{Y-p}_2
\end{align*}
\end{theorem}
\begin{proof}
\begin{align*}
\prob{Y\neq \sign[\bfw.\bfX] }=\frac{1}{2} - \frac{1}{2}\<Y,\sign[\bfw.\bfX]\>
\end{align*}

\begin{lem}
Given $\gamma, \tau>0$, there exists a polynomial $p_{\gamma, \tau}$ of degree $O(\frac{1}{\gamma}\log \frac{1}{\tau})$ such that
\begin{itemize}
\item For any $x\in [-1,1]$, $|p_{\gamma, \tau}(x)\leq (1+\tau)$.
\item For any $x\in [-1,1]$ with $|x|>\gamma$, $|p_{\gamma, \tau}(x)-\sign(x)|<\tau.$
\end{itemize}
\end{lem}



\begin{align*}
\<Y,\sign[\bfw.\bfX]\> &= \<Y, p_{\gamma}(\bfw.\bfX)\> + \<Y,(p_{\gamma}(\bfw.\bfX)- \sign[\bfw.\bfX])\>\\
& = \<\Pi_Y^\gamma, p_{\gamma}(\bfw.\bfX)\> + \<Y,(p_{\gamma}(\bfw.\bfX)- \sign[\bfw.\bfX])\>\\
&\leq \norm{\Pi_Y^\gamma}_1 \norm{p_{\gamma}}_{\infty, [-1,1]} + \norm{p_{\gamma} - \sign}_{1, D_w}\\
&\leq \norm{\Pi_Y^\gamma}_1 (1+\tau) + \norm{p_{\gamma} - \sign}_{1, D_w}
\end{align*}



\begin{align*}
\norm{p_{\gamma} - \sign}_{1, D_w}& =\PP(|\bfw.\bfX|> \gamma ) \EE[\big| p_{\gamma}(\bfw.\bfX) - \sign(\bfw.\bfX)\big|~|\bfw.\bfX|> \gamma ]\\
&~~ +\PP(|\bfw.\bfX|\leq \gamma ) \EE[\big| p_{\gamma}(\bfw.\bfX) - \sign(\bfw.\bfX)\big|~|\bfw.\bfX|\leq  \gamma ]\\
& \leq \tau +  \PP(|\bfw.\bfX|\leq \gamma ) (2+\tau)
\end{align*}
\begin{fact}
Let $\bfX$ be a random variable with uniform distribution on $\SS^{d-1}$. Then, for any vector $\bfw\in \RR^d$ with $\sum_{i}w_i^2=1$ and any $\gamma \in [0,1]$, we have 
\begin{align*}
\prob{|\bfw.\bfX| \leq \gamma} = 2\frac{A_{d-2}}{A_{d-1}} \int_0^\gamma (1-z^2)^{\frac{d-3}{2}}dz \leq \gamma O(\sqrt{d}).
\end{align*}
\end{fact}

Let $\tau = \epsilon'$ and $\gamma =  O(\frac{\epsilon'}{\sqrt{d}})$ so that 
\begin{align*}
\norm{p_{\gamma} - \sign}_{1, D_w} \leq 2\epsilon'.
\end{align*}
With that 
\begin{align*}
\<Y,\sign[\bfw.\bfX]\> \leq  \norm{\Pi_Y^{\epsilon'}}_1 (1+\epsilon') +2\epsilon'.
\end{align*}
and 
\begin{align*}
\prob{Y\neq \sign[\bfw.\bfX] } \geq \frac{1}{2} - \frac{ 1+\epsilon'}{2}\norm{\Pi_Y^{\epsilon'}}_1 - \epsilon'. 
\end{align*}

\end{proof}
\begin{theorem}\label{thm:low degree concentrated}
Let $D$ be a joint probability distribution with marginal $D_X$ that is uniform over $\SS^{d-1}$. Let $\mathcal{C}$ be the set of all linear threshold functions on $\SS^{n-1}$. Then, for any $\delta\in[0,1]$, with probability at least $1-\delta$, the $\Ltwo$-polynomial regression algorithm agnostically PAC learns $\mathcal{C}$ with generalization error upto 
 \begin{align*}
\prob{Y\neq \predict(\bfX)}\leq 2 \Pek+O\Big(\sqrt{\frac{\lambda(k)}{n}\log\frac{d}{\delta}}\Big),
\end{align*}
where $\lambda(k)=k^2 2^{2k} c_k^{2}$, with $c_k\deq \max_{\mathcal{S}\subseteq [d], |\mathcal{S}|\leq k} \norm{\pS}_{\infty}^2$. 
\end{theorem}



\begin{proof}
 \begin{align*}
\Pemp\Big\{Y\neq \hat{g}(\bfX)\Big\} &\leq  \frac{1}{2}\Big(2-2\norm{\hat{p}}_{1,\Demp}\Big)\leq 2\Pekemp+2\epsilon,
\end{align*}
\end{proof}

==> fourier.tex <==
\section{Fourier Analysis in Product Probability Spaces}\label{app:Fourier_analysis}
The following facts summarize some basic properties of the Fourier expansion. These statements are derived from the orthogonality of the parities. Hence, we omit the proofs. 
\begin{fact}\label{fact:fourier1}
For any bounded pair of functions $f,g: \pmm^d\mapsto \RR$, the following statements hold: 
\begin{itemize}
\item Plancherel Identity: $\EE[f(\bfX)g(\bfX)]=\sum_{\mathcal{S}\subseteq [d]} \fS g_{\mathcal{S}}$. 
\item Parseval’s identity $\norm{f}_2^2=\sum_{\mathcal{S}\subseteq [d]} \fS^2$.
\item Jensen's Inequality: $\norm{f}_1\leq \norm{f}_2$.
%\item If the image of $f,g$ is $\pmm$, then $\PP\big\{f(X^d)\neq g(X^d)\big\}= \frac{1}{4}\norm{f-g}_2^2.$
\end{itemize}
\end{fact}

\begin{fact}\label{fact:fourier_boolean}
Let $f:\pmm^d\mapsto \pmm$ and $\mathcal{J}\subseteq [d]$, then the following holds
\begin{itemize}
\item $\norm{f}_1=\norm{f}_2=1$ and $\norm{\fJ}_2\leq 1$.
\item $ \norm{\fJ}_2^2 \leq   \norm{\fJ}_1 \leq \norm{\fJ}_2$. 
\end{itemize}
\end{fact}

\begin{fact}\label{fact:2norm and fJ}
If $g:\pmm^d\mapsto \pmm$ is a function whose output depends only on the coordinates of a subset $\mathcal{J}\subseteq [d]$, then $g_{\mathcal{S}}=0$ for all $\mathcal{S}\nsubseteq \mathcal{J}$. Further,  for any $f: \pmm^d \mapsto \pmm$
\begin{align*}
\norm{f -g}_2^2 = 1 - \norm{\fJ}_2^2 + \norm{\fJ - g}_2^2 
\end{align*}
\end{fact}
\begin{fact}\label{fact:mismatch norm2}
Given a joint distribution $D$ on $\mathcal{X}\times \pmm$, the misclassification probability of any prediction functions $g: \mathcal{X}\mapsto \pmm$ can be written as 
\begin{align*}
\prob{Y\neq g(\bfX)}=\frac{1}{2}-\frac{1}{2}\<Y,g\> = \frac{1}{4}\norm{Y-g}_2^2.
\end{align*}
\end{fact}
%In the next lemma, we show an identity between the misclassification 
%probability and the Fourier coefficients.
%\begin{lem}\label{lem:misclassifican_fourier_XZ}
%Consider a pair of finite sets $\mathcal{X}$ and $\mathcal{Z}$ with elements in $\RR$, and  a joint probability distribution $P_{X,Z}$ with marginals $P_X$ and $P_Z$. Suppose $(X_i,Z_i), i\in[d]$ are a sequence of IID random variables each distributed according to $P_{X,Z}$. Then, for functions $f: \mathcal{X}^d \mapsto \pmm$, and $g: \mathcal{Z}^d\mapsto \pmm$ we have that 
%$$\PP\Big\{f(X^d)\neq g(Z^d)\Big\}= \frac{1}{2}-\frac{1}{2}
%\sum_{\mathcal{S}\subseteq [d]} \fS ~{g}_{\mathcal{S}} ~\rho^{|\mathcal{S}|} .$$
%where $\rho$ is the correlation coefficient between $X$ and $Z$. Moreover, $\fS$ are the Fourier coefficients of $f$ with respect to the product probability space  $\Pspace$ and $\tilde{g}_{\mathcal{S}}$ are the Fourier coefficients of $g$  with respect to the product probability space  $(\mathcal{Z}^d, P_{\mathcal{Z}^d})$. 
%\end{lem}
%We finish this review with a statement of the Azuma's inequality.





==> proof_kjuntaappx.tex <==
\section{Proof of Theorem \ref{thm:kjunta_nonbinary}}\label{proof:kjunta_nonbinary}
\begin{proof}
From Lemma \ref{lem:misclassifican_fourier_XZ}, for any $g:\mathcal{X}^k\mapsto \pmm$  the mismatch probability satisfies
\begin{equation}\label{eq:k-junta:mismatch}
\prob\{f(\bfX ) \neq g(\bfX)\}   = \frac{1}{2} - \frac{1}{2} \sum_{S \in [n]} \hat{f}_S ~ \hat{g}_S,
\end{equation}
where $\hat{f}_S, \hat{g}_S$ are the Fourier coefficients of $f$ and $g$, respectively.
Suppose that $g(\bfx)$ is a $k$-junta and depends only on the inputs $(x_i)_{i\in J}$, where $J$ is a subset of $[n]$ with at most $k$ elements. Then, $\hat{g}_S=0$ for any $S \nsubseteq J$. Hence, from the definition of the projection $\fJ$, the mismatch probability in \eqref{eq:k-junta:mismatch} equals 
%
\begin{align}
%
\nonumber
 \prob\{f(\bfX ) \neq g(\bfX)\}   &= \frac{1}{2} - \frac{1}{2}\<f^{\subseteq J},g \>\\ 
&   \geq \frac{1}{2} - \frac{1}{2}\<  \abs{f^{\subseteq J}}, \abs{g} \> =   \frac{1}{2} - \frac{1}{2} \|f ^{\subseteq J} \|_1.
%
\label{eq:k-junta:mismatch 2}
\end{align}
%
The last equality in Equation \eqref{eq:k-junta:mismatch 2} holds because $|g(\bfx)|=1$ for all $\bfx\in \mathcal{X}^d$. Since $J$ is an arbitrary subset of $[n]$ with at most $k$ elements, Equation \eqref{eq:k-junta:mismatch 2} implies
 %
\begin{align}
\label{eq:Pek_lb}
 \Pek[f] \geq \frac{1}{2}-\frac{1}{2} \max_{J\subseteq [n], \,  \abs{J} \leq k} \|f^{\subseteq J}\|_1.
\end{align}
%

Next we obtain an upper bound on  $\Pek[f]$ by specifying a $k$-junta approximation of $f$.  Fix a subset  $J\subseteq [n]$ with $|J|\leq k$, and let $g=\sign[f^{\subseteq J}]$. Note that for any $f$ we have 
%
\begin{align} 
%
\nonumber
\<g, f^{\subseteq J}\> & = \expec[ f^{\subseteq J}(\bfx) \cdot \sign[f^{\subseteq J}(\bfx)] ] \\
% 
& = \EE[ \, \abs{f^{\subseteq J}(\bfx)} \, ]  =\|f^{\subseteq J}\|_1. \label{eq:innerL1}
%
\end{align} 
%
Therefore, using \eqref{eq:k-junta:mismatch 2}, the mismatch probability of this approximation is
\begin{equation}
\prob(f(\bfX ) \neq g(\bfX))=  \frac{1}{2}-\frac{1}{2}\|f^{\subseteq J}\|_1.
\label{eq:mis_achieve}
\end{equation}
Eq. \eqref{eq:mis_achieve}  provides an upper-bound on $ \Pek[f]$ for any $J$ such that $\abs{J} \leq k$. Taking $J=J^*$, where $J^*$ achieves $ \max_{J\subseteq [n], \,  \abs{J} \leq k}\|f^{\subseteq J}\|_1$, we obtain
%
 \begin{equation}
 %
 \Pek[f]  \leq  \frac{1}{2}-\frac{1}{2} \max_{J\subseteq [n], \,  \abs{J} \leq k} 
 \|f^{\subseteq J}\|_1.
 \label{eq:pekub}
 \end{equation}
 Combining \eqref{eq:pekub} and \eqref{eq:Pek_lb} completes the proof.
 \end{proof}
\begin{corollary}\label{corr:bounds on mismatch}
The minimum mismatch probability satisfies
\begin{align}
& \frac{1}{2}\left[  1-\max_{J\subseteq [1,n], \,  \abs{J} \leq k}\|f^{\subseteq J}\|_2 \right] 
\nonumber  \\
 &\quad \leq  \Pek[f] \leq  \frac{1}{2}\left[ 1-\max_{J\subseteq [1,n],~ |J|\leq k}\|f^{\subseteq J}\|^2_2\right],
\end{align}
\end{corollary}
%
\begin{proof}
%
Since $\fJ(x^d)=\EE[f(X^d)|x^J]$, then $-1\leq f^{\subseteq J}\leq 1$ which implies that $|f^{\subseteq J}(\bfx)|\geq |f^{\subseteq J}(\bfx)|^2 $. Thus $\|f^{\subseteq J}\|_1\geq \|f^{\subseteq J}\|^2_2$, which yields the upper bound by substituting in \eqref{eq:minimum_mismatch_prob}.
Next, from Jensen's inequality we have
\begin{equation*}
\EE\Big[|f^{\subseteq J}(\bfX)|^2\Big] \geq  \Big[ \EE \abs{f^{\subseteq J}(\bfX)}\Big]^2.
\end{equation*}
This implies that $\|f^{\subseteq J}\|_2 \geq \|f^{\subseteq J}\|_1$, which establishes the lower-bound.
\end{proof}


==> proof_lem_2norm_projection.tex <==
\section{Proof of Lemma \ref{lem:2norm and projection}}\label{app:proof of lem 2norm projection}

By adding and subtracting  $\fJ$ we have 
\begin{align*}
\norm{f-\hJ}_2^2 &= \norm{T_f + (\fJ-\hJ)}_2^2\\
&\stackrel{(a)}{=}\<(T_f + (\fJ-\hJ)), (T_f + (\fJ-\hJ))\> \\ \numberthis \label{eq:norm T_f}
&\stackrel{(b)}{=} \norm{T_f}_2^2 + \norm{\fJ-\hJ}_2^2
\end{align*}


From the definition of the projection function $\fJ$, the inner product $\<Y-\fJ, \pS\> = 0$ for any $\mathcal{S}\subseteq \mathcal{J}$. Therefore,
\begin{align*}
\<T_f, \hJ\> = \sum_{\mathcal{S}\subseteq \mathcal{J}} h_{\mathcal{S}}~ \<T_f, \pS\> = 0.
\end{align*}
Similarly, $\<T_f, \fJ\> =0$. Thus, by adding and subtracting  $\fJ$ we have 
\begin{align*}
\norm{f-\hJ}_2^2 &= \norm{T_f + (\fJ-\hJ)}_2^2\\
&\stackrel{(a)}{=}\<(T_f + (\fJ-\hJ)), (T_f + (\fJ-\hJ))\> \\ \numberthis \label{eq:norm T_f}
&\stackrel{(b)}{=} \norm{T_f}_2^2 + \norm{\fJ-\hJ}_2^2
\end{align*}
where $(a)$ is due to the identity $\norm{g}_2^2 = \<g,g\>$ and $(b)$ is due the orthogonality of $T_f$ and $(\fJ-\hJ)$. Similarly, we obtain that 
\begin{align}\label{eq:2norm f and T_f}
\norm{f}_2^2 = \norm{T_f+\fJ}_2^2 = \norm{T_f}_2^2 + \norm{\fJ}_2^2.
\end{align}
Lastly, the proof is complete by combining \eqref{eq:norm T_f} and \eqref{eq:2norm f and T_f}.

==> proof_lem_imscore.tex <==
\section{Proof of Lemma \ref{lem:imscore and 1norm}}\label{proof:lem_imscore}

\begin{proof}
We apply Azuma's inequality for $\score_1(\mathcal{J})$ which is a 
function of the random training samples. The constants $c_i$, 
as in Lemma \ref{lem:Azuma}, for this function are equal to 
$$\frac{4}{n-1}2^k \max_{\mathcal{S}\subseteq[d], 
|\mathcal{S}|\leq k}\norm{\pS}_{\infty}^2 \deq \frac{4~2^k c_k}{n-1}.
$$
From Azuma's inequality, for a fixed subset $\mathcal{J}\subseteq [d]$ with $|\mathcal{J}|= k$ 
\begin{align*}
\prob{ \big|\score_1(\mathcal{J})-\EE[\score_1(\mathcal{J})]   
\big|\leq \epsilon'}\leq 2\exp\Big\{-\frac{(n-1)\epsilon'^2}{32~2^{2k}c_k^2} \Big\}.
\end{align*}
Hence, using the union bound, the inequalities 
$$\big|\score_1(\mathcal{J})-\EE[\score_1(\mathcal{J})]  
\big|\leq \epsilon', \quad \forall \mathcal{J}\subseteq [d],~ |\mathcal{J}|= k
$$
hold with probability $(1-\delta_2)$ provided that $(n-1)\geq \tilde{n}(\epsilon,\delta)$, where 
$$\tilde{n}_2(\epsilon',\delta_2)= \frac{32~2^{2k}c_k^2}{\epsilon'^2} 
\log\Big(\frac{{d\choose k}}{2\delta}\Big).
$$ 
Next, from Lemma \ref{lem:score_1 unbiased}, we have that
\begin{align}\label{eq:Azuma_score_1}
\Big| \EE\big[\score_1(\mathcal{J})\big]-  \norm{\fJ}_1  \Big| &\leq \frac{2^{k/2}}{\sqrt{n-1}}.
\end{align}

Lastly, we combine this inequality to the one in \meqref{eq:Azuma_score_1}. 
That said, from the triangle inequality, we have that
$$\big|\score_1(\mathcal{J})-\norm{\fJ}_1\big|\leq \epsilon'+\frac{2^{k/2}}{\sqrt{n-1}}, 
\quad \forall \mathcal{J}\subseteq [d],~ |\mathcal{J}|= k
$$
hold with probability $(1-\delta_1)$ provided that 
$n\geq \tilde{n}(\epsilon',\delta_1)+1$. Hence, setting 
$\epsilon_1=\epsilon'+\frac{2^{k/2}}{\sqrt{n-1}}$ and 
$n_1(\epsilon_1, \delta_1)=\tilde{n}(\epsilon',\delta_1)+1$ complete the proof. 
\end{proof}


==> proof_lem_norm2sign.tex <==
\section{Proof of Lemma \ref{lem:norm2 sign}}\label{app:proof norm2 sign}


From \eqref{eq:error and inner prod} in the main text, the generalization error of $\sign[\hJ]$ can be written as $\frac{1}{2}-\frac{1}{2}\<Y,\sign[\hJ]\>$. Since $\sign[\hJ]$ is a function depending only on the coordinates of $\mathcal{J}$, then in the inner product, we can replace $Y$ with $\PiJ$. Hence, we obtain that
\begin{align}\nonumber
\PP\Big\{Y\neq  \sign[
\hJ(\bfX)]\Big\} &= \frac{1}{2}-\frac{1}{2}\<\PiJ,\sign[\hJ]\>\\\label{eq:pe 2 norm stoch}
 &= \frac{1}{4}\big(1-\norm{\PiJ}_2^2+\norm{\PiJ-\sign[\hJ]}_2^2\big).
\end{align}
   The $2$-norm quantity above is upper-bounded as follows
\begin{align*}
 \norm{\PiJ-\sign[\hJ]}_2^2  &\stackrel{(a)}{\leq} \Big(\norm{\PiJ-\hJ}_2+\norm{\hJ-\sign[\hJ]}_2\Big)^2,\\\numberthis \label{eq:mismatch_2norm}
 &= \Big(\norm{\PiJ-\hJ}^2_2+\norm{\hJ-\sign[\hJ]}^2_2+2\norm{\PiJ-\hJ}_2\norm{\hJ-\sign[\hJ]}_2 \Big),
\end{align*}
where $(a)$  follows from the Minkowski's Inequality inequality for $2$-norm.  Note that  $|\hJ-\sign[\hJ]|= |1-\hJ|.$ Therefore,
\begin{align}\nonumber
\norm{\hJ-\sign[\hJ]}^2_2&=\EE\left[(1-|\hJ({X^{\mathcal{J}}})|)^2\right]\\\label{eq:fbar-sign}
&= 1+\norm{\hJ}_2^2-2\norm{\hJ}_1.
\end{align}
From this relation and equations \eqref{eq:pe 2 norm stoch},  \meqref{eq:mismatch_2norm}, we obtain the following upper bound
\begin{align}\nonumber
4\PP\Big\{Y\neq \sign[
\hJ(\bfX)]\Big\} &\leq 2-2\norm{\hJ}_1+ \underbrace{ \norm{\hJ}_2^2- \norm{\PiJ}_2^2}_{\text{(I)}}\\\label{eq:up1}
&~~+\norm{\PiJ-\hJ}^2_2 +2\norm{\PiJ-\hJ}_2\underbrace{\norm{\hJ-\sign[\hJ]}_2}_{\text{(II)}}. 
\end{align}
In what follows, we bound the terms denoted by (I) and (II).
\paragraph{Bounding (I):} From the Minkowski's inequality for $2$-norm, we have
\begin{align*}
\norm{\hJ}_2^2 &\leq \Big(\norm{\PiJ}_2+\norm{\hJ-\PiJ}_2  \Big)^2\\
&=\norm{\PiJ}^2_2+\norm{\hJ-\PiJ}^2_2+2\norm{\PiJ}_2 \norm{\hJ-\PiJ}_2\\
&\leq \norm{\PiJ}^2_2+{\norm{\hJ-\PiJ}^2_2+2 \norm{\hJ-\PiJ}_2}
\end{align*}
where the second inequality is due Bessel's inequality implying that $\norm{\PiJ}_2\leq 1$. Hence, the term (I) in \meqref{eq:up1} is upper bounded as
\begin{align}\label{eq:bound on (I)}
\text{(I)}\leq \lambda_1\deq \norm{\hJ-\PiJ}^2_2+2 \norm{\hJ-\PiJ}_2.
\end{align}


\paragraph{Bounding (II):} From \meqref{eq:fbar-sign}, we have
\begin{align*}
\norm{\hJ-\sign[\hJ]}_2^2 &= 1+\norm{\hJ}_2^2-2\norm{\hJ}_1\\
&\stackrel{(a)}{\leq} 1+ 2( \norm{\PiJ}^2_2+ \norm{\PiJ-\hJ}^2_2)-2\norm{\hJ}_1\\
&\stackrel{(b)}{=} 1+ 2( \norm{\PiJ}^2_2+ \norm{\PiJ-\hJ}^2_2)-2\big(\norm{\PiJ}_1+ ( \norm{\hJ}_1-\norm{\PiJ}_1)\big)\\
&= 1+ 2( \norm{\PiJ}^2_2- \norm{\PiJ}_1)+ 2 \norm{\PiJ-\hJ}^2_2-2\big( \norm{\hJ}_1-\norm{\PiJ}_1\big)\\
&\stackrel{(c)}{\leq}  1+ 2 \norm{\PiJ-\hJ}^2_2-2\big( \norm{\hJ}_1-\norm{\PiJ}_1\big)\\\numberthis \label{eq:temp1}
&\stackrel{(d)}{\leq } 1+ 2 \norm{\PiJ-\hJ}^2_2+2\norm{\PiJ-\hJ}_2,
\end{align*}
where $(a)$ follows from the Minkowski's inequality for $2$-norm and the inequality $(x+y)^2\leq 2(x^2+y^2)$. Equality $(b)$ follows by adding and subtracting  $\norm{\PiJ}_1$. Inequality $(c)$ holds, since from Jensen's inequality $ \norm{\PiJ}^2_2\leq  \norm{\PiJ}_1$. Lastly, inequality $(d)$ holds because of the following chain of inequalities
\begin{align}\label{eq:normdiff_leq_eps}
\Big|\norm{\PiJ}_1-\norm{\hJ}_1\Big| \leq \norm{\PiJ-\hJ}_1\leq \norm{\PiJ-\hJ}_2,
\end{align}
where the first inequality is due to the Minkowski's inequality for $1$-norm and 
the second inequality is due to Holder's inequality. 

Next, we show that the quantity $\big\| \hJ-\sign[h_\mathcal{J}]\big\|_2$ without the square is upper bounded by the same term as in the right-hand side of \meqref{eq:temp1}. That is 
\begin{align}\label{eq:bound on (II)}
\text{(II)} &= \big\| \hJ-\sign[h_\mathcal{J}]\big\|_2\leq \lambda_2\deq 1+ 2 \norm{\PiJ-\hJ}^2_2+2\norm{\PiJ-\hJ}_2.
\end{align}
The argument is as follows: if $\big\| \hJ-\sign[h_\mathcal{J}]\big\|_2$  is 
less than one, then the upper bound holds trivially as $\lambda_2\geq 1$; 
otherwise, this quantity is less than its squared and, hence, the upper-bound holds.  

As a result of the bounds in \meqref{eq:up1}, \eqref{eq:bound on (I)}, and \eqref{eq:bound on (II)} we obtain that 
\begin{align*}
4\PP\Big\{Y \neq \sign[\hJ(\bfX)]\Big\}  &\leq 2-2\norm{\hJ}_1+ \lambda_1+\norm{\PiJ-\hJ}^2_2+  2 \lambda_2 \norm{\PiJ-\hJ}_2\\
&= 2-2\norm{\PiJ}_1+\Big(\norm{\PiJ}_1-\norm{\hJ}_1\Big)  +\lambda_1+\norm{\PiJ-\hJ}^2_2+ 2 \lambda_2 \norm{\PiJ-\hJ}_2\\
&\leq 2-2\norm{\PiJ}_1+\norm{\PiJ-\hJ}_2+ \lambda_1+\norm{\PiJ-\hJ}^2_2+  2 \lambda_2 \norm{\PiJ-\hJ}_2,
\end{align*}
where the last inequality is due to \meqref{eq:normdiff_leq_eps}. Therefore, from the definition of $\lambda_1$ and $\lambda_2$, and the function $U$ in the statement of the lemma, we obtain 
\begin{align*}
4\PP\Big\{Y\neq \sign[
\hJ(\bfX)]\Big\}  \leq 2-2\norm{\PiJ}_1+4U(\norm{\PiJ-\hJ}_2).
\end{align*}
This completes the proof.



==> proof_score_unbiased.tex <==
\section{Proof of Lemma \ref{lem:score_1 unbiased}}\label{proof:lem:score1 unbiased}
\begin{proof}
We start with rewriting $\score_1$. Define, the function
\begin{align}\label{eq:FestJi}
\FestJi (\bfx)\deq \frac{n}{n-1} \sum_{\mathcal{S} \subseteq \mathcal{J}} \Big( \FestS-\frac{1}{n}Y(i)\prod_{j\in \mathcal{S}} \frac{X_j(i)-\hat{\mu}_j}{\hat{\sigma}_j}\Big)  \pestS(\bfx),
\end{align}
for all $x\in \pmm^d$. With this definition, given any $\bfx$, the quantity $\FestJi (\bf)$ is independent of $(X^d(i),Y(i))$. Further, we can write $\score_1$ as the summation $\score_1(\mathcal{J})=\frac{1}{n}\sum_i |\FestJi (\bfX(i))|$. Hence,  the exception of $\score_1$ taken over the training samples gives 
\begin{align*}
\EE[\score_1(\mathcal{J})]&=\frac{1}{n}\sum_{i=1}^n \EE_{\bfX(1),..., \bfX(n)}\Big[~\Big|~\FestJi (\bfX(i))~\Big|~\Big]\\
&=\EE_{\bfX(1),..., \bfX(n)}\Big[~\Big|~\FestJone (\bfX(1))~\Big|~\Big]\\
&=\EE_{\bfX(2),..., \bfX(n)}\EE_{\bfX(1)}\Big[~\Big|~\FestJone (\bfX(1))~\Big|~\Big]\\\numberthis \label{eq:E score_1}
&=\EE_{\bfX(2),..., \bfX(n)}\big[\norm{\FestJone}_1\big],
\end{align*}
where the first equality is due to the symmetry with respect to the index $i$ of the training samples.  The last equality is due to  the definition of $1$-norm and the property that the function $\FestJone$ is independent of $(\bfX(1),Y(1))$. 
Note that $\FestJone$ is as an estimation of the projection $\fJ$ using the $(n-1)$ training samples $(\bfX(i),Y(i)), i=2,3,..., n$. Next, we bound the difference $\Big|\EE\norm{\FestJone}_1 - \norm{\fJ}_1\Big|$. 
Observe that 
\begin{align*}
\Big| \EE\big[\norm{\FestJone}_1\big]-  \norm{\fJ}_1  \Big| &\leq \EE\big[\norm{\fJ-\FestJone}_1\big]\\
&\leq \EE\big[\norm{\fJ-\FestJone}_2\big]\\
&\leq \sqrt{\EE\big[\norm{\fJ-\FestJone}^2_2\big]}
\end{align*}
where the first inequality is obtained by applying the triangle inequality twice, one for $\norm{\FestJone}_1$ and once for $\norm{\fJ}_1$. The second inequality is from the identity $\norm{\cdot }_1\leq \norm{\cdot}_2$ as in Fact \ref{fact:fourier1}. The third inequality is due to the Jensen's inequality.
Note that as $\hat{\mu}_j=\mu_j$ and $\hat{\sigma}_j=\sigma_j$, then $\pestS\equiv \pS$. Therefore, by Parseval's identity in Fact \ref{fact:fourier1}, we have
\begin{align*}
\EE\big[\norm{\fJ-\FestJone}^2_2\big]&=\sum_{S\subseteq J} \EE\big[|\fS-\FestSone|^2\big]=\sum_{S\subseteq J} \operatorname{var}\big(\FestSone\big).
\end{align*}
Note that $\FestSone$ is the empirical average of \ac{IID} random variables $Y(i)\pS(\bfX(i))$ for $i=2,3,...,n$. Thus,  
\begin{align*}
\operatorname{var}\big(\FestSone\big)&=\frac{1}{n-1}\operatorname{var}\big(Y\pS(\bfX)\big)\\
&=\frac{1}{n-1}(\EE\big[Y^2\pS^2(\bfX)\big]-\fS^2)\\
&=\frac{1}{n-1}(1-\fS^2),
\end{align*}
where the last equality holds because of of the following chain of equalities: 
\begin{align*}
\EE\big[Y^2\pS^2(\bfX)\big]=\EE\big[\pS^2(\bfX)\big]= \<\pS, \pS\> = 1,
\end{align*}
where the first equality holds because $Y^2=1$ which is due to the fact that $Y\in \pmm$. The last equality is due to orthonormality of the parities. 

As a result of the above argument, we can write 
\begin{align*}
\EE\big[\norm{\fJ-\FestJone}^2_2\big]&=\frac{1}{n-1}\sum_{S\subseteq J} (1-\fS^2)=\frac{1}{n-1}(2^{|\mathcal{J}|}-\norm{\fJ}_2^2)\\
&\leq \frac{1}{n-1}2^k
\end{align*}
Putting all together we get that 
\begin{align*}
\Big| \EE\big[\norm{\FestJone}_1\big]-  \norm{\fJ}_1  \Big| &\leq \frac{2^{k/2}}{\sqrt{n-1}}
\end{align*}
The proof is complete by the above inequality and \meqref{eq:E score_1}. 








\end{proof}

==> proof_thm_norm2.tex <==
\section{Proof of Theorem \ref{thm:alg2_norm2}}\label{proof:thm alg2_norm2}
For the simplicity of the proof, it is assumed that $\bar{\mu}_j=\mu_j$ and $\bar{\sigma_j}=\sigma_j$.
Let $\Jalgb$ be the the selected feature subset in the algorithm. By $\mathcal{J}^*_2$ denote the feature subset that maximizes the $2$-norm $\norm{\fJ}_2$ among all subsets of size at most $k$.  Then, we have
\begin{align*}
\prob{f(X^d)\neq \sign[\falgb(X^{\Jalgb})]}&\leq \norm{f-\falgb}_2^2\\
&=1-\norm{\fJalgb}_2^2+\norm{\fJalgb-\falgb}_2^2,
\end{align*}
where the inequality is due to the fact that $\11\big\{ f(x^d)\neq \sign[\falgb(x^{\Jalgb})]\big\}\leq \big(f(x^d)-\falgb(x^{\Jalgb}) \big)^2$.
Next, we apply Lemma \ref{lem:fbarJbar-fJbar} in Subsection \ref{subsec:technical}. Fix $\epsilon, \delta\in (0,1)$ and suppose the sample size is at least $n_2(\epsilon, \delta)$ as in the lemma. Then, with probability at least $(1-\delta)$, we have  $\norm{\fJalgb-\falgb}_2^2\leq \epsilon^2$. Hence, 
\begin{align}\nonumber
\prob{f(X^d)\neq \sign[\falgb]}&\leq  1-\norm{\fJalgb}_2^2 +\epsilon^2\\\label{eq:norm2 bound on Pe}
&= 1-\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2 + \Big( \underbrace{\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2- \norm{\fJalgb}_2^2}_{\text{(I)}}\Big) +\epsilon^2
\end{align}
Next, we show that the term (I) in the last equality is sufficiently small.  From the triangle inequality for $2$-norm, we have for any subset $\mathcal{J}$ that
\begin{align*}
\norm{\festJ}_2^2&\leq \Big(\norm{\fJ}_2+\norm{\festJ-\fJ}_2  \Big)^2\\
&=\norm{\fJ}^2_2+\norm{\festJ-\fJ}^2_2+2\norm{\fJ}_2 \norm{\festJ-\fJ}_2\\\numberthis \label{eq:2norm_festJ-fJ} 
&\leq \norm{\fJ}^2_2+\norm{\festJ-\fJ}^2_2+2 \norm{\festJ-\fJ}_2,
\end{align*}
where the last inequality holds as $\norm{\fJ}_2 \leq 1$.
Therefore, applying Lemma \ref{lem:fbarJbar-fJbar}, we obtain, with probability at least $(1-\delta)$ that $$\norm{\festJ}_2^2- \norm{\fJ}^2_2 \leq \epsilon^2+2\epsilon$$
The above inequality also implies that $\norm{\festJ}_2^2 \leq 1+\epsilon^2+2\epsilon\leq 4$. Hence using a similar argument as in \meqref{eq:2norm_festJ-fJ}, we get that 
\begin{align*}
\norm{\fJ}_2^2-\norm{\festJ}_2^2 \leq \epsilon^2 + 8\epsilon.
\end{align*}
As a result, noting  $\epsilon^2\leq \epsilon$, we obtain that $\big| ~\norm{\festJ}_2^2- \norm{\fJ}^2_2~\big| \leq 9\epsilon$. Note that $\score_2(\mathcal{J})=\norm{\festJ}_2^2$. Therefore, for any feature subset $\mathcal{J}$ with size $k$ the inequalities
\begin{align*}
\Big| \score_2(\mathcal{J})-\norm{\fJ}_2^2~\Big|\leq 9\epsilon
\end{align*}
hold with probability at least $(1-\delta)$. Thus, from the above inequalities and the fact that $\Jalgb$ maximizes $\score_2$, we have 
\begin{align*}
\norm{\fJalgb}_2^2 &\geq \score_2(\Jalgb)-9\epsilon\\
&\geq \score_2(\mathcal{J}^*_2)-9\epsilon\\
&\geq \norm{f^{\subseteq \mathcal{J}^*_2}}_2^2 -18\epsilon
\end{align*}
Therefore, term (I) in \meqref{eq:norm2 bound on Pe} is at most $18\epsilon$ and we get 
\begin{align*}
\prob{f(X^d)\neq \sign[\falgb]}&\leq 1-\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2 +\epsilon^2+18\epsilon.
\end{align*}
Note from \meqref{eq:2norm_Pkf} that $\norm{f^{\subseteq \mathcal{J}^*_2}}_2 \geq 1-2\P^k[f]$. Therefore, 
\begin{align*}
\prob{f(X^d)\neq \sign[\falgb]}&\leq 1-(1-2\P^k[f])^2 +\epsilon^2+18\epsilon\\
&= 4\P^k[f]-4(\P^k[f])^2 +\epsilon^2+18\epsilon.
\end{align*}
This completes the proof. 

==> proof_thm_regret.tex <==
\section{Proof of Theorem \ref{thm:regret}}\label{app:proof thm regret}
Note that $\predict \equiv \sign[ \falg]$ and by $\Peg$ denote its misclassification probability.   Then, from Lemma \ref{lem:norm2 sign}, we have that 
\begin{align*}
\Peg \deq \PP_{\bfX,Y}\{Y\neq  \predict(\bfX^{\Jalg})\} \leq \frac{1}{2}(1-\norm{\fJalg}_1)+U(\norm{\fJalg-\falg}_2),
\end{align*}
where $U$ is a polynomial of the form $U(x)=x^3+\frac{3}{2}x^2+\frac{5}{4}x$. Taking the expectation with respect to the training samples $\mathcal{D}_n$ gives, 
\begin{align*}
\EE_{\mathcal{D}_n}[\Peg] \leq \frac{1}{2}(1-\EE_{\mathcal{D}_n}[\norm{\fJalg}_1])+\EE_{\mathcal{D}_n}[U(\norm{\fJalg-\falg}_2)].
\end{align*}
Therefore, subtracting $\Pek$ gives 
\begin{align*}
\EE_{\mathcal{D}_n}[\Peg]-\Pek &\leq \frac{1}{2}(1-\EE_{\mathcal{D}_n}[\norm{\fJalg}_1])+\EE_{\mathcal{D}_n}\big[U(\norm{\fJalg-\falg}_2)\big] - \Pek\\\numberthis \label{eq:P-P_opt}
&=\frac{1}{2} \underbrace{(\norm{\fJstar}_1-\EE_{\mathcal{D}_n}[\norm{\fJalg}_1])}_{\text{(I)}}+\underbrace{\EE_{\mathcal{D}_n}\big[U(\norm{\fJalg-\falg}_2)\big]}_{\text{(II)}}.
\end{align*}
 Next, we provide upper bounds for the terms (I) and (II). 


\paragraph{Bounding (I):} 
Note that $\Jalg$ is a feature subset maximizing $\imscore_1$ as in \eqref{eq:1norm_est}. Whereas, $\mathcal{J}^*$ maximizes $\norm{\fJ}_1$.  Therefore, by adding and subtracting $\EE[\imscore_1(\Jalg)]$ and $\EE[\imscore_1(\mathcal{J}^*)]$ we have:
\begin{align*}
\text(I) &=\big( \norm{\fJstar}_1 - \EE[\imscore_1(\mathcal{J}^*)]\big) + \big(\EE[\imscore_1(\mathcal{J}^*)] - \EE[\imscore_1(\Jalg)]\big)\\
&\quad + \big(\EE[\imscore_1(\Jalg)]- \EE[\norm{\fJalg}_1]\big)\\
&\stackrel{(a)}{\leq} \EE\big[ \norm{\fJstar}_1 - \imscore_1(\mathcal{J}^*)\big] +  \EE\big[\imscore_1(\Jalg)-\norm{\fJalg}_1\big]\\
& \leq 2 \max_{\mathcal{J}: |\mathcal{J}|=k} \big|\EE[\imscore_1(\mathcal{J})]- \norm{\fJ}_1\big|\\\numberthis \label{eq:reg term I up}
&\stackrel{(b)}{\leq} O(n^{-\gamma}),
\end{align*}
where  $(a)$ holds as $\imscore_1(\Jalg)\geq \imscore_1(\mathcal{J}^*)$ and inequality $(b)$ follows from Lemma \ref{lem:score_1 unbiased adjusted} with $\gamma\in (0,1/2)$.
\paragraph{Bounding (II):} 
We start by removing the effect of $\Jalg$ by maximizing over all feature subsets $\mathcal{J}$:
\begin{align*}
\text{(II)} \leq \max_{\mathcal{J}: |\mathcal{J}|=k} \EE_{\mathcal{D}_n}\big[U(\norm{\fJ-\hat{f}^{\subseteq \mathcal{J}}}_2)\big]
\end{align*}
Fix a $k$-element subset $\mathcal{J}\subseteq [d]$ and let $Z\deq \norm{\fJ-\hat{f}^{\subseteq \mathcal{J}}}_2$. Note that $Z$ is a random variables which is a function of the training samples $\mathcal{D}_n$.  From Lemma \ref{lem:fbarJbar-fJbar} we know that given $\epsilon_2, \delta_2$, the inequality $\PP\{Z> \epsilon_2\}\leq \delta_2$ holds if $n\geq n_2(\epsilon_2, \delta_2)$, where $n_2(\cdot)$ is defined in the lemma. Therefore, by conditioning on the event $\{Z \leq \epsilon_2\}$ and its complement, we have
\begin{align*}
\EE\big[U(Z)\big] &= \PP\big\{Z \leq \epsilon_2 \big\}\EE\big[U(Z)\big| Z\leq \epsilon_2\big] + \PP\big\{Z>\epsilon_2\big\} \EE\big[U(Z)\big| Z>\epsilon_2\big]\\
&\stackrel{(a)}{\leq} \EE\big[U(Z)\big|Z\leq \epsilon_2 \big] + \delta_2 \EE\big[U(Z)\big| Z>\epsilon_2\big]\\
&\stackrel{(b)}{\leq} U(\epsilon_2 ) + \delta_2 \EE\big[U(Z)\big| Z>\epsilon_2\big]\\\numberthis \label{eq:EU(Z) up}
&\stackrel{(c)}{\leq} U(\epsilon_2 )  + \delta_2 \max_{(\bfx(i), y(i))} U(\norm{\fJ-\hat{f}^{\subseteq \mathcal{J}}}_2), 
\end{align*}
where $(a)$ is due to the inequalities $\PP\{Z \leq \epsilon_2 \} \leq 1$ and $\PP\{Z> \epsilon_2\}\leq \delta_2$.  Inequality $(b)$ holds due to the conditioning $Z\leq \epsilon_2$ and the fact that $U$ is a monotone function. Inequality $(c)$ follows by replacing the expectation with maximization  over all realizations of the training samples. Next, we upper-bound the term inside $U(\cdot)$. From the triangle inequality, we obtain  that 
\begin{align*}
\norm{\fJ-\hat{f}^{\subseteq \mathcal{J}}}_2\leq  \norm{\fJ}_2 + \norm{\hat{f}^{\subseteq \mathcal{J}}}_2 \leq  1 +  \norm{\hat{f}^{\subseteq \mathcal{J}}}_{\infty},
\end{align*}
where  the last inequality holds due to $\norm{\fJ}_2 \leq 1$ and the identity  $\norm{\cdot}_2 \leq \norm{\cdot}_\infty$. Not that $\hat{f}^{\subseteq \mathcal{J}}\equiv \sum_{\mathcal{S}\subseteq \mathcal{J}}  \festS \pestS$ and that the Fourier coefficients $\festS$ can be written as a linear combination of the parities as in \eqref{eq:emp fourier coeff}.  Hence, from the definition of $\norm{\cdot}_{\infty}$, we obtain that
\begin{align*}
\norm{\hat{f}^{\subseteq \mathcal{J}}}_{\infty} = \max_{\bfx} \big|\hat{f}^{\subseteq \mathcal{J}}(\bfx)\big|\leq \big| \sum_{\mathcal{S}\subset \mathcal{J}} \norm{\pS}_{\infty}^2\big|\leq 2^k c_k,
 \end{align*} 
where $c_k$ is the same term as in Theorem \ref{thm:unknownf_and_D}. 
As a result of the above equations and \eqref{eq:EU(Z) up}, we get the upper bound $\EE[U(Z)]  \leq  U(\epsilon_2 )  + \delta_2 ~ (1+2^k c_k)$. Since this bound is independent of the choice of the $k$-element subset $\mathcal{J}$, then the inequality
\begin{align*}
\text{(II)} \leq U(\epsilon_2 )  + \delta_2 ~ U(1+2^k c_k). 
\end{align*}
holds as long as $n\geq n_2(\epsilon_2, \delta_2)$. 
\paragraph{Tuning $(\epsilon_2, \delta_2)$: }
Now let $\gamma\in (0, \frac{1}{2})$ and set 
\begin{align*}
\epsilon_2 = 2^{k/4} n^{-\gamma}, \qquad \delta_2 = 2kd^k\exp\{\frac{-n^{1-2\gamma}}{8c_k}\}.
\end{align*}
With this choice $n_2(\epsilon_2, \delta_2) = n$. Further, we obtain in the following that
\begin{align*}
\text{(II)} \leq U(2^{k/4}  n^{-\gamma} )  +  2kd^kU(1+2^k c_k)\exp\{\frac{-n^{1-2\gamma}}{8c_k}\} \stackrel{(a)}{=} O(n^{-\gamma} ),
\end{align*}
where $(a)$ holds, since the exponential term on the left-hand side converges to zero faster than $n^{-\gamma}$. 
Consequently, from the above equation, \eqref{eq:reg term I up}, and the inequality \eqref{eq:P-P_opt}, we get
\begin{align*}
\EE_{\mathcal{D}_n}[\Peg]-\Pek  \leq O(n^{-\gamma}) + O(n^{-\gamma}) = O(n^{-\gamma}).
\end{align*}
 This completes the proof. 

==> twoNorm.tex <==
\subsection{Replacing $1$-norm with $2$-norm}
To reduce the computational complexity, we can use 
the 2-norm expression $\norm{\fJ}^2_2$, 
instead of the $1$-norm expression in Algorithm~\ref{alg:feature_selection}. As for the theoretical justification of $2$-norm, we have the following lemma.
\begin{lem}\label{lem:P_k[f]- 2-norm}
The minimum attainable misclassification probability  satisfies the following inequalities
 \begin{align}\label{eq:2norm_Pkf}
 \frac{1}{2}\big(  1-\max_{\mathcal{J}:~ |\mathcal{J}|=k}~ \norm{\fJ}_2 \big)
 \leq  \Pek \leq   \frac{1}{2}\big( 1-\max_{\mathcal{J}:~ |\mathcal{J}|=k} ~\norm{\fJ}_2^2\big).
\end{align}
\end{lem}
\begin{proof}
We first prove the lower-bound. From Proposition \ref{prop:kjunta_nonbinary}, $\Pek$ can be written as
\begin{align*}
 \Pek&=\frac{1}{2}-\frac{1}{2}\norm{\fJstar}_1
 \end{align*} 
where $J^*=\argmax_{\mathcal{J}: |\mathcal{J}|\leq k} \norm{\fJ}_1$. From Fact \ref{fact:fourier_boolean} of Appendix \ref{app:Fourier_analysis}, we obtain that $$\norm{\fJstar}_1\leq \norm{\fJstar}_2\leq \max_{\mathcal{J}: |\mathcal{J}|\leq k} \norm{\fJ}_2.$$ 
This establishes the lower bound. As for the upper bound, for any $k$-element subset $\mathcal{J}\subseteq [d]$, we have
\begin{align*}
 \Pek&\leq \frac{1}{2}-\frac{1}{2}\norm{\fJ}_1 \leq \frac{1}{2}-\frac{1}{2}\norm{\fJ}_2^2
 \end{align*} 
 where the first inequality follows as $\norm{\fJstar}_1\geq \norm{\fJ}_1$, and the last inequality follows from Fact \ref{fact:fourier_boolean}. Since the last inequality holds for any subset $\mathcal{J}$ of size $k$, we can take the minimum of the right-hand side. This establishes the upper-bound and completes the proof.
\end{proof}
  For the feature selection in this approach, 
the algorithm searches for the feature subset $\mathcal{J}$ 
that maximizes the estimate of the $2$-norm. Due to Parseval's identity the $2$-norm satisfies $\norm{\fJ}_2^2 =  \sum_{\mathcal{S} \subseteq \mathcal{J}} \fS^2$. Hence, %the $2$-norm can be computed as  $\norm{\fJ}_2^2 = \sum_{\mathcal{S} \subseteq \mathcal{J}} \fS^2$.  To 
to estimate it we use 
\begin{align}\label{eq:score2}
\imscore_2(\mathcal{J}) = \widehat{\norm{\fJ}^2_2} \deq  \sum_{\mathcal{S} \subseteq \mathcal{J}} \bigg(\frac{1}{n}\sum_{i=1}^n\Big[ y(i)~ \prod_{j\in \mathcal{S}} \frac{x_j(i)-\hat{\mu}_j}{\hat{\sigma}_j}\Big]\bigg)^2.
\end{align}
With this modification, in line 3 and 4 of Algorithm \ref{alg:feature_selection} we replace $\score_1$ with $\score_2$. One can show that the low degree algorithm is a special case of our algorithm when the features are known to be uniform over $\pmm^d$. 

 To make sure that $\score_2$ is an accurate enough estimate of $\norm{\fJ}_2^2$ fewer training samples are required compared to $\score_1$. However, the theoretical guarantees for universality no longer hold for this measure. Instead, we prove weaker but useful theoretical justifications for using $2$-norm. In particular, we show in the following theorem that misclassification probability of the new algorithm is at most  $2\Pek(1-\Pek)$. The proof of the theorem is provided in Subsection \ref{subsec:roadmap 2 norm}.
 
\begin{theorem}\label{thm:alg2_norm2}
If $\score_1$ in Algorithm \ref{alg:feature_selection} is replaced by $\score_2$, then for any $\delta, \epsilon \in (0,1)$ and labeling functions $f$, the new misclassification rate is at least  $\big(2\Pek(1-\Pek)+\epsilon\big)$, with 
probability at least $(1-\delta)$, provided that the training 
sample size is atleast $n(\epsilon, \delta)$ as in Theorem \ref{thm:unknownf_and_D}.
\end{theorem}
%Computing $\score_2(\mathcal{J})$ for a fixed subset $\mathcal{J}$ with cardinality $k$ takes $O(nk2^k)$ arithmetic operations. The  Therefore, comparing to $\score_1$, we obtain a polynomial-time (of order $n$) reduction in computational complexity.
%% A sufficient  sample complexity to calculate this score for $m$ different feature subsets is given in  the following lemma.
%\begin{lem}
%For $\epsilon, \delta\in (0,1)$,  a sequence of feature subsets $\clJ_1, \clJ_2, \cdots, \clJ_m$, and $n$ randomly generated training samples, the inequalities
%\begin{align*}
%\Big|\imscore_2(\clJ_i)-\score_2(\clJ_i)\Big|\leq \epsilon,
%\end{align*}
%hold for all $i\in [m]$ and with probability at least $(1-\delta)$, provided that 
%$$n\geq \frac{c_m}{\epsilon^2}\log_2\big(\frac{2m}{\delta}\big),$$
%where $c_m$ is a constant depending on the sequence of the feature subsets an is bounded by $2^{O( \max_i |\clJ_i|)}$. 
% \end{lem}  
%
%
%As a result, with the exhaustive search over all feature subsets of size at most $k$ the required samples complexity is $\frac{1}{\epsilon^2} {2^{O(k)}}\log_2\big(\frac{2k d^k}{\delta}\big)$.
%




%Once such a feature subset is found, the predictor is obtained by 
%estimating the corresponding projection and taking its sign.
%We call it Algorithm 2. 
%(see Algorithm \ref{alg:conventional search alg}).   
\begin{comment}
\begin{algorithm2e}[ht]
\caption{Fourier-Based Learning with a Greedy Search Algorithm}
\label{alg:conventional search alg}
\DontPrintSemicolon
\LinesNumbered

\KwIn{$k, d, n$, and the training samples $(\bfx(1), y(1)), (\bfx(2), y(2)), \cdots, (\bfx(n), y(n))$}
\KwOut{Feature subset $\Jalgb$, and the predictor $\predictb$}
 \SetKwProg{Est}{Greedy Feature Selection}{:}{\KwRet $\Jalgb$}
 \SetKwProg{Prd}{Predictor}{:}{\KwRet $\predictb$}
Compute the empirical mean $\hat{\mu}_j$ and standard deviation $\hat{\sigma}_j$ of each feature $j=1,2, ...,d$. \;
 \Est{}{ 
Run greedy search algorithm with the scoring function $\imscore_2$ defined in 
Equation \eqref{eq:score2}.\; 
 Set $\Jalgb$ as the best found feature subset\;}
\Prd{}{
Compute the empirical Fourier coefficients $\festS$, as in Equation \eqref{eq:emp fourier coeff}, for all $\mathcal{S}\subseteq \Jalg$.\;
Construct  the empirical projection function $\falgb$ defined as  $$\falgb(\bfx) \deq \sum_{\mathcal{S}\subseteq \Jalgb }    \festS\prod_{j\in \mathcal{S}} \frac{x_j-\hat{\mu}_j}{\hat{\sigma}_j}.$$ 
Construct the predictor  as $\predictb=\sign[\falgb]$.\;
}
\end{algorithm2e}
\end{comment}



\subsection{Steps for Proving Theorem \ref{thm:alg2_norm2}}\label{subsec:roadmap 2 norm}
Let $\Jalgb$ be the the selected feature subset in the algorithm with $\imscore_2$. With that, the algorithm outputs the predictor  $\predict_2 \equiv \sign[\fJalgb]$. Therefore, the resulted misclassification probability of the algorithm with $\imscore_2$ is denoted by 
\begin{align*}
\Pegb = \prob{Y\neq \predict_2(\bfX^{\Jalgb})}.
\end{align*}
Our objective is to derive the bound on the sample size $n$ so that $\Pegb\leq \big(2\Pek(1-\Pek)+\epsilon\big)$, with probability at least $(1-\delta)$.  The proof of Theorem  \ref{thm:alg2_norm2} is given in three steps. 




\paragraph{Step 1. ( Characterization of the mislcassification probability ):}
We start with an upper bound on the misclassification probability. From Lemma \ref{lem:norm2 sign}, we have 
\begin{align*}
\Pegb &\leq \frac{1}{2}(1-\norm{\fJalgb}_1) + U(\norm{\fJalgb - \falgb}_2),\\
&\leq \frac{1}{2}(1-\norm{\fJalgb}_2^2) + U(\norm{\fJalgb - \falgb}_2),
\end{align*}
where the last inequality follows from the inequality $\norm{\cdot}_2^2 \leq \norm{\cdot}_1$ as stated in Fact \ref{fact:fourier_boolean} of Appendix \ref{app:Fourier_analysis}.

By $\mathcal{J}^*_2$ denote the feature subset that maximizes the $2$-norm expression below
\begin{align*}
\mathcal{J}^*_2 \deq \argmax_{\mathcal{J}\subseteq [d]: |\mathcal{J}|=k} \norm{\fJ}_2.
\end{align*}

Next, by adding and subtracting  $\frac{1}{2}\norm{f^{\subseteq \mathcal{J}^*_2}}_2^2$, we obtain that
\begin{align}\label{eq:Pegb 2norm}
\Pegb \leq \frac{1}{2}\Big(1-\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2\Big) + \frac{1}{2}\Big( \underbrace{\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2- \norm{\fJalgb}_2^2}_{\text{(I)}}\Big) + U\Big( \underbrace{\norm{\fJalgb-\falgb}_2^2}_{\text{(II)}}\Big).
 \end{align}
Here, the effect of the feature selection on the misclassification probability is presented by the term (I). Also, the effect of the accuracy of the estimations is indicated by the term (II). In what follows, we analyze these terms. 

\paragraph{Step 2 (Accuracy of the Estimations):} 
It follows by Lemma \ref{lem:fbarJbar-fJbar} 
that the inequality 
$\norm{\fJ - \festJ}_2 \leq \epsilon_2$ holds for all $k$-element subsets 
$\mathcal{J}$ with probability at least $(1-\delta_2)$ when at 
least $n_2(\epsilon_2, \delta_2)$ (as in Lemma \ref{lem:fbarJbar-fJbar})
number of training samples are available. 
As a result, the term (II) satisfies 
\begin{align*}
\norm{\fJalgb-\falgb}_2^2 \leq \epsilon^2_2,
\end{align*}
with probability atleast $(1-\delta_2)$. 

\paragraph{Step 3 (Effect of the Feature Selection):}

Next, we show that the term (I) is sufficiently small.  From the triangle inequality for $2$-norm, we have for any subset $\mathcal{J}$ that
\begin{align*}
\norm{\festJ}_2^2&\leq \Big(\norm{\fJ}_2+\norm{\festJ-\fJ}_2  \Big)^2\\
&=\norm{\fJ}^2_2+\norm{\festJ-\fJ}^2_2+2\norm{\fJ}_2 \norm{\festJ-\fJ}_2\\\numberthis \label{eq:2norm_festJ-fJ} 
&\leq \norm{\fJ}^2_2+\norm{\festJ-\fJ}^2_2+2 \norm{\festJ-\fJ}_2,
\end{align*}
where the last inequality holds as $\norm{\fJ}_2 \leq 1$.
Therefore, applying Lemma \ref{lem:fbarJbar-fJbar}, we obtain, with probability at least $(1-\delta
_2)$ that $$\norm{\festJ}_2^2- \norm{\fJ}^2_2 \leq \epsilon_2^2+2\epsilon_2.$$
The above inequality also implies that $\norm{\festJ}_2^2 \leq 1+\epsilon_2^2+2\epsilon_2\leq 4$. Hence using a similar argument as in \meqref{eq:2norm_festJ-fJ}, we get that 
\begin{align*}
\norm{\fJ}_2^2-\norm{\festJ}_2^2 \leq \epsilon_2^2 + 8\epsilon_2.
\end{align*}
As a result, noting  $\epsilon_2^2\leq \epsilon_2$, we obtain that $\big| ~\norm{\festJ}_2^2- \norm{\fJ}^2_2~\big| \leq 9\epsilon_2$. Note that $\score_2(\mathcal{J})=\norm{\festJ}_2^2$. Therefore, for any feature subset $\mathcal{J}$ with size $k$ the inequalities
\begin{align*}
\Big| \score_2(\mathcal{J})-\norm{\fJ}_2^2~\Big|\leq 9\epsilon_2
\end{align*}
hold with probability at least $(1-\delta_2)$. Thus, from the above inequalities and the fact that $\Jalgb$ maximizes $\score_2$, we have 
\begin{align*}
\norm{\fJalgb}_2^2 &\geq \score_2(\Jalgb)-9\epsilon_2\\
&\geq \score_2(\mathcal{J}^*_2)-9\epsilon_2\\
&\geq \norm{f^{\subseteq \mathcal{J}^*_2}}_2^2 -9\epsilon_2
\end{align*}
Therefore, term (I) in \meqref{eq:Pegb 2norm} is at most $9\epsilon_2$ and we get 
\begin{align*}
\Pegb &\leq \frac{1}{2}\Big(1-\norm{f^{\subseteq \mathcal{J}^*_2}}^2_2\Big) +9\epsilon_2+U(\epsilon_2^2).
\end{align*}
Note that from \meqref{eq:2norm_Pkf}, we get the inequality $\norm{f^{\subseteq \mathcal{J}^*_2}}_2 \geq 1-2\Pek$. Therefore, 
\begin{align*}
\Pegb &\leq \frac{1}{2}\big(1-(1-2\Pek)^2\big) +9\epsilon_2+U(\epsilon_2^2)\\
&= 2\Pek-2(\Pek)^2+9\epsilon_2+U(\epsilon_2^2).
\end{align*}
This completes the proof. 
